FORML: A Riemannian Hessian-free Method for Meta-learning on Stiefel Manifolds

Meta-learning problem is usually formulated as a bi-level optimization in which the task-specific and the meta-parameters are updated in the inner and outer loops of optimization, respectively. However, performing the optimization in the Riemannian space, where the parameters and meta-parameters are located on Riemannian manifolds is computationally intensive. Unlike the Euclidean methods, the Riemannian backpropagation needs computing the second-order derivatives that include backward computations through the Riemannian operators such as retraction and orthogonal projection. This paper introduces a Hessian-free approach that uses a first-order approximation of derivatives on the Stiefel manifold. Our method significantly reduces the computational load and memory footprint. We show how using a Stiefel fully-connected layer that enforces orthogonality constraint on the parameters of the last classification layer as the head of the backbone network, strengthens the representation reuse of the gradient-based meta-learning methods. Our experimental results across various few-shot learning datasets, demonstrate the superiority of our proposed method compared to the state-of-the-art methods, especially MAML, its Euclidean counterpart.

==> Sections/Abstract.tex <==
\begin{abstract}
  Many methods formulate the Meta-learning problem as a bi-level optimization in which the task-specific and the meta-parameters are updated in the inner and outer loops of optimization, respectively. However, performing the optimization in the Riemannian space, where the parameters and meta-parameters are located on Riemannian manifolds is computationally intensive. Unlike the Euclidean methods, backpropagation needs computing the second-order derivatives that include backward computations through the Riemannian operators such as retraction and orthogonal projection. In this paper, we introduce a Hessian-free approach that uses a first-order approximation of derivatives.          
\end{abstract}

==> Sections/Conclusion.tex <==
\section{Conclusion}
\label{Sec-Conclusion}
sss

==> Sections/Introduction.tex <==
\section{Introduction}
\label{Sec-Introduction}
Meta-learning has attracted growing attention recently, owing to its capability to learn from several tasks and generalize to unseen ones. From the Optimization-based point of view, meta-learning can be formulated as a bi-level optimization problem, consisting of two optimization levels. At the outer level, a meta-learner extracts the meta-knowledge (the \textit{how to learn } knowledge) from specific tasks, whereas at the inner level, each specific task is learned via a base-learner. Among different approaches to meta-learning, in optimization-based methods (please refer to ) the meta-learner \textit{learn how to optimize} the task-specific base learners. In other words, both the meta and base learners are (usually gradient descent) optimizers. Then the meta-knowledge can be considered as the step-size, gradient, or anything that can affect or improve the inner-level optimizers. 

In practice, numerous learning tasks are modeled as optimization problems with nonlinear constraints. For instance, many classic machine learning problems such as Principal component analysis (PCA) \cite{yuan2019online}, independent component analysis (ICA) \cite{hyvarinen2000independent} and subspace learning \cite{chakraborty2020intrinsic} are cast as optimization problems with orthogonality constraints. Also, modern deep neural networks benefit from applying the orthogonality constraint on their parameter matrices, which results in significant advantages such as increasing the accuracy and attaining a faster convergence rate \citep{bansal2018can}, improving the generalization \citep{cogswell2015reducing} and stabilizing the distribution of neural activations during the training of Convolutional Neural Networks (CNNs) \citep{huang2018building}. A popular way to incorporate nonlinear constraints into optimization frameworks is to make use of Riemannian geometry and formulate constrained problems as optimization on Riemannian manifolds \cite{lin2008riemannian}. In this case, Euclidean meta-learning with nonlinear constraints is cast as meta-learning on Riemannian manifolds, namely learning to optimize in Riemannian spaces. To do so, the optimization algorithm should be respectful to the Riemannian geometry, which can be achieved by utilizing the Riemannian operations such as \textit{retraction, orthogonal projection} and \textit{parallel transport}. However,  learning optimizers on Riemannian manifolds need second-order differentiation through the nonlinear Riemannian optimization, which is complex and computationally expensive.

In this paper, we propose a Riemannian meta-optimization method that uses a first-order approximation to calculate the derivatives. In the inner loop of our algorithm, base learners are optimized using a limited number of steps on the Riemannian manifold. At the outer loop, to update the meta-optimizer, instead of computing the derivatives through the entire inner-level path, they are computed by only considering the last step of the inner-level optimization. In this way, learning the meta-optimizer does not need to differentiate through the complex Riemannian optimization in the inner loop. Therefore, our method avoids the exploding gradient issue caused by computing products of Hessian and gradients of the retraction, resulting in computational efficiency and stability of the bi-level optimization. We empirically show that our proposed method can be trained efficiently and learn a good optimization trajectory compared to other methods.

The rest of the paper is organized as follows. Section~\ref{Sec-Preliminaries} covers the common foundations on which we will base our proposed algorithms. Section~\ref{Sec-method} describes our proposed technique,~\textit{i.e} First Order Riemannian Meta-Learning (FORML) methods. The experimental analysis, evaluations, and results are presented in Section~\ref{Sec-Results}. Finally, Section~\ref{Sec-Conclusion} concludes the paper.


==> Sections/Method.tex <==
\section{Proposed Method}
\label{Sec-method}
Generally, the optimization-based meta-training (learn to optimize) on Riemannian manifolds can be formulated as \cite{tabealhojeh2023rmaml}:
\begin{align}
     \label{Eq:general-Riemannian-meta-train}
\bm{\theta}_{meta}^*= \underbrace{\min_{\bm{\theta}\in\Manifold}{\frac{1}{N} \sum_{i=1}^{N}{\Loss_{i}\big(\bm{\Dataset}_i^{q},\overbrace{\bm{\phi}_{i}^{*}}^{\text{inner-level}})}}}_{\text{outer-level}}\big) 
\end{align}

where $N$ is the number of training tasks, $\bm{\theta}$ and $\bm{\phi}$ respectively indicate the meta-parameters and parameters of the meta-learner that are located on a Riemannian manifold $\Manifold$, ~\textit{i.e} $\bm{\theta}, \bm{\phi}\in\Manifold$. $\Loss_i$ is the loss function of the $i^{th}$ task, whereas $\Dataset_i=\{\bm{\Dataset}_i^{s},\bm{\Dataset}_i^{q}\}$ demonstrates the meta-train dataset of $i^{th}$ task. The support set $\bm{\Dataset}_i^{s}$ and the query set $\bm{\Dataset}_i^{q}$ are respectively analogous to training and validation datasets in classic supervised training. Eqn.~\eqref{Eq:general-Riemannian-meta-train} demonstrate two levels of optimization. The outer loop (or the meta-optimizer) learns the optimal meta-parameter, ~\textit{i.e} $\bm{\theta}_{meta}^*$ using query datasets from a distribution of $N$ training tasks and the optimal task-specific parameters $\bm{\phi}_{i}^*$. However, as the $\bm{\phi}_{i}^*$ is unknown, it can be solved as another optimization problem (the inner-level optimization). Therefore, Eqn.~\eqref{Eq:general-Riemannian-meta-train} can be considered as a bilevel optimization; a constrained optimization in which each constraint is itself an optimization problem:                    
\begin{align}
    \label{Eq:bi-level-Riemannian}
    \begin{split}
\bm{\theta}_{meta}^*=\min_{\bm{\theta}\in\Manifold}{\frac{1}{N} \sum_{i=1}^{N}{\Loss_{i}\big(\bm{\Dataset}_i^{q},\bm{\phi}_i^*\big)}}
 \\ 
 \text{subject to}~~\bm{\phi}_i^*=\gfun(\bm{\Dataset}_i^{s},\bm{\theta}_{meta}^*)
\end{split}
\end{align}

Where $\gfun(\bm{\Dataset}_i^{s},\bm{\theta}_{meta}^*)$ is (usually) a gradient descent optimizer which is dependent on the meta-knowledge, $\bm{\theta}_{meta}^*$. The meta-knowledge can be interpreted as learning an appropriate parameter initialization \cite{tabealhojeh2023rmaml} or even learning to optimize a LSTM model \cite{gao2020learning,gao2022learning}. Assuming the meta-parameter as an initial point, the bilevel optimization problem of qn.~\eqref{Eq:bi-level-Riemannian}, can be solved by performing two nested loops. At the inner loop, a limited number of gradient descent steps are performed to optimize each task-specific parameter $\bm{\phi}_i^*$ using the meta-parameter as an initial point,~\textit{i.e} $\bm{\phi}_i^{(0)}=\bm{\theta}_{meta}$, and the outer loop performs a gradient descent update for the meta-parameter, $\bm{\theta}_{meta}$.  Each step of the inner loop optimization problem can be formulated as follows: 

\begin{equation}
\begin{aligned}
\label{eqn:task_specific_params_rmaml}
\bm{\phi}_i^{(l+1)}=
R_{\bm{\phi}_i^{(l)}}\left(-\alpha \pi_{\bm{\phi}_i^{(l)}}\left(\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})\right)\right), l\ge 1
\end{aligned}    
\end{equation}
in which the Euclidean gradient vector $\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})$ is projected to the tangent space of $\bm{\phi}_i^{(l)}$ and then the parameters are updated by performing the \textit{retraction} operator {$R_{\bm{\phi}_i^{(l)}}$}.

Moreover, a single step of gradient decent in Riemannian space for the outer loop is as follows:
%\begin{equation}
%\begin{aligned}
%\label{eqn:rmaml_2}
%\bm{\theta}^{(t+1)}=\\
%R_{\bm{\theta}^{(t)}}\left(-\beta \left( \sum_{\Tau_i \in \Tau}\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}^{(t)}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)\right)\right)  
%\end{aligned}    
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\label{eqn:rmaml_2}
%\bm{\theta}_{meta}^*=\\
%R_{\bm{\theta}}\left(-\beta \left( \sum_{\Tau_i \in \Tau}\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)\right)\right)  
%\end{aligned}    
%end{equation}
%\HT{where for each task, the projected gradient vector is parallely transported from the tangent space of $\bm{\phi}_i$ (\textit{i.e.} $\bm{\phi}_i^{(k)}$ using $k$ inner-level updates) to the tangent space of the current meta-parameter $\bm{\theta}^{(t)}$. Thus, the meta-parameter is updated by performing the \textit{retraction} operator $R_{\bm{\theta}^{(t)}}$. Equivalently Eqn.~\eqref{eqn:rmaml_2} can be written as follows}:
%\begin{align}
%\label{eqn:rmaml_1}
%\bm{\theta}_{meta}^*= R_{\bm{\theta}}\left(-\beta \sum_{\Tau_i \in \Tau}{\pi_{\bm{\theta}}}\Big(\nabla_{\bm{\theta}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)\right)     
%\end{align}
\begin{align}
\label{eqn:rmaml_1}
\bm{\theta}^{(t+1)}= R_{\bm{\theta}^{(t)}}\left(-\beta \sum_{i=1}^{M}{\pi_{\bm{\theta}^{(t)}}}\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)\right)     
\end{align}
where to calculate $\bm{\theta}^{(t+1)}$, the Euclidean gradient vector of each task, $\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$ is orthogonally projected to the tangent space of the current meta-parameter by $\pi_{\bm{\theta}^{(t)}}(.)$ operation. Then the summation over the Riemannian gradient of all the tasks is retracted to the manifold. To compute the gradient vector $\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$
For each task, differentiating through the inner-level optimization path is needed. In other words, calculating $\pi_{\bm{\theta}^{(t)}}\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$ requires a gradient of the gradients and needs a heavy computation for the second-order derivatives that include backward computations through the Riemannian operators such as retraction and orthogonal projection. Assuming that $k$ Riemannian gradient descent steps are performed in the inner level optimization, then: 

\begin{align}
\label{eqn:derivatives}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)= \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)     
\end{align}

where $\bm{\phi}_i^{(k)}$ is the result of inner-level optimization:
\begin{gather}    
\label{eqn:derivatives2}
\bm{\phi}_i^{(k)}=
R_{\bm{\phi}_i^{(k-1)}}\left(-\alpha \pi_{\bm{\phi}_i^{(k-1)}}\left(\nabla_{\bm{\phi}_i^{(k-1)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(k-1)})\right)\right)\\
\bm{\phi}_i^{(k-1)}=
R_{\bm{\phi}_i^{(k-2)}}\left(-\alpha \pi_{\bm{\phi}_i^{(k-2)}}\left(\nabla_{\bm{\phi}_i^{(k-2)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(k-2)})\right)\right)\\
\vdots \\
\bm{\phi}_i^{(0)}=\bm{\theta}^{(t)}  
\end{gather}

Thus, the derivative in the Eqn.~\eqref{eqn:derivatives} becomes as follows:

\begin{align}
\label{eqn:derivatives3}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
= \frac{\partial \Loss_i}{\partial \bm{\phi}_i^{(k)}}\frac{\partial \bm{\phi}_i^{(k)}}{\partial \bm{\theta}^{(t)}}
\end{align}

in which the $\frac{\partial \bm{\phi}_i^{(k)}}{\partial \bm{\theta}^{(t)}}$ term can be further unfolded as follows:

\begin{gather}
\label{eqn:derivatives5}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
= \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)}{\partial \bm{\phi}_i^{(k)}} \prod_{l=1}^{k}{  \frac{\partial \bm{\phi}_i^{(l)}}{\partial \bm{\phi}_{i}^{(l-1)}}}\\
= \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)}{\partial \bm{\phi}_i^{(k)}} \prod_{l=1}^{k}{\frac{\partial \bigg( R_{\bm{\phi}_i^{(l-1)}}\left(-\alpha \pi_{\bm{\phi}_i^{(l-1)}}\left(\nabla_{\bm{\phi}_i^{(l-1)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l-1)})\right)\right)\bigg)}{\partial \bm{\phi}_{i}^{(l-1)}}}
\end{gather}

For simplification, let us consider exactly one update at the inner level. Thus this step of inner-level optimization is as follows:

\begin{align}
\label{eqn:derivatives6}
    \bm{\phi}_i^{(1)}=
R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}_i^{(t)})\right)\right)
\end{align}

Therefore, the Eqn.~\eqref{eqn:derivatives5} is as follows:
\begin{align}
    \label{eqn:derivatives7}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    =\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}} \frac{\partial \bigg( R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)}{\partial \bm{\theta}^{(t)}}
\end{align}

The above expression is general for Riemannian manifolds. For instance, considering the Euclidean manifold, the  Eqn.~\eqref{eqn:derivatives7} can be computed as below:
\begin{align}
    \label{eqn:derivatives8}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    =\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}} \frac{\partial \bigg( \bm{\theta}^{(t)}-\alpha (\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\bigg)}{\partial \bm{\theta}^{(t)}}
\end{align}

which can be further simplified as:
\begin{align}
    \label{eqn:derivatives9}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    =\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}  \bigg( \bm{I}-\alpha (\nabla^{2}_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\bigg)
\end{align}

\subsection{First Order approximation: From Euclidean space to Stiefel manifold}
For the Euclidean spaces, the first-order approximation of Eqn.~\eqref{eqn:derivatives3} can be calculated by ignoring the second-order derivatives of Eqn.~\eqref{eqn:derivatives9}:
\begin{align}
    \label{eqn:derivatives9}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    =\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}
\end{align}

  On the other hand, calculating such an approximation for the Riemannian spaces is not straightforward. In the rest of the section, we derive the formulation of first-order approximation on Stiefel manifolds. To do so, we compute the $\frac{\partial \bigg( R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)}{\partial \bm{\theta}^{(t)}}$ term of the Eqn.~\eqref{eqn:derivatives7}:

  \begin{gather}
    \label{eqn:derivatives10}
    d\bigg(R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)=d\bigg( \bm{\theta}^{(t)}-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right) \bigg)
    \\=d(\bm{\theta}^{(t)})-d\bigg(\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right) \bigg)
    \\=d(\bm{\theta}^{(t)})-\alpha d\bigg( \nabla_{\bm{\theta}^{(t)}}-\bm{\theta}^{(t)}\frac{(\bm{\theta}^{(t)})^{T} \nabla_{\bm{\theta}^{(t)}}- (\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)}}{2} \bigg)\\
    = I-\alpha d(\nabla_{\bm{\theta}^{(t)}})+0.5\alpha d\bigg( \bm{\theta}^{(t)} (\bm{\theta}^{(t)})^{T} \nabla_{\bm{\theta}^{(t)}}\bigg)-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)} \bigg)\\
    =I-\alpha d(\nabla_{\bm{\theta}^{(t)}})+0.5\alpha d\bigg( \nabla_{\bm{\theta}^{(t)}}\bigg)-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)} \bigg)\\
    =I-0.5\alpha d(\nabla_{\bm{\theta}^{(t)}})-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)} \bigg)\\
    = I-0.5\alpha d(\nabla_{\bm{\theta}^{(t)}})-0.5\alpha d(\bm{\theta}^{(t)})(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)}-0.5\alpha \bm{\theta}^{(t)}d(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)}-0.5\alpha \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T}d(\bm{\theta}^{(t)})
\end{gather}
Obviously, the second and forth terms of above formula contain second-order derivatives. By ignoring those terms, we have:
\begin{gather}
 \label{eqn:derivatives11}
  -0.5\alpha vec( d(\bm{\theta}^{(t)})(\nabla_{\bm{\theta}^{(t)}})^{T}\bm{\theta}^{(t)})-0.5\alpha vec(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T}d(\bm{\theta}^{(t)}))\\
  =-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}})\otimes I\bigg) vec( d(\bm{\theta}^{(t)})-0.5\alpha\bigg(I\otimes \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T} \bigg) vec( d(\bm{\theta}^{(t)})\\
  =-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}})\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T} \bigg)vec( d(\bm{\theta}^{(t)})
\end{gather}

altogether we will have:
\begin{align}
    \label{eqn:derivatives12}
    d\bigg(R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)\approx I-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}})\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T} \bigg)
\end{align}
finally:
\begin{align}
    \label{eqn:derivatives13}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    \approx\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}\bigg(I-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}})\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}})^{T} \bigg) \bigg)
\end{align}
%\begin{align}
%\label{eqn:rmaml_new}
%\bm{\theta}^{(t+1)}= R_{\bm{\theta}^{(t)}}\left(-\beta \sum_{i=1}^{M}%{\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)}\right)    %
%\end{align}

 %where $\pi_{\bm{\theta}} \Big(\nabla_{\bm{\theta}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$=$\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right) $
\subsection{The proposed bi-level algorithm}
The full proposed method is outlined in Algorithm~\ref{alg-RMAML}. Practically we meta-optimize the last fully-connected layer of the backbone network using FORML on Stiefel manifold, while the other parameters are optimized on Euclidean space. Moreover, we normalize the input of the Stiefel layer. As a result, the forward computation of that fully-connected layer acts as a Cosine distance between the input vector $\textbf{x}$ and the weight vectors of the classes that are columns of the weight matrix $\textbf{W}$. (As shown in Figure~\ref{fig:Stiefel-layer}.  
\begin{align}
    \label{eqn:Stiefel layer}
    \textbf{W}^{T}\textbf{x}=\frac{\textbf{W}^{T}\textbf{x}}{\| \textbf{W} \| \| \textbf{x} \|}=\gamma
\end{align}

\begin{algorithm*}
\centering
\caption{RMAML}\label{alg-RMAML}
\begin{algorithmic}[1]
\Require %Distribution over meta-training tasks $p(\Tau)$, inner-level learning rate $\alpha$, outer-level learning rate $\beta$.

$p(\Tau)$ denotes the distribution over meta-training tasks.

~~~$\alpha$ denotes the inner-level learning rate.

~~~$\beta$ represents the outer-level learning rate.
\vspace{0.1cm}
%\Require Inner-level learning rate $\alpha$, outer-level learning rate $\beta$.
\vspace{0.1cm}
\State Randomly initialize  $\bm{\theta}^{(0)}$
\vspace{0.1cm}
% \State \SR{What about $\bm{\theta}$ and not $\bm{\theta}_{meta}$??}
\While{not done}
    \vspace{0.1cm}
    \State Sample batch $\{\Tau_i\}_{i=1}^B$ 
    \vspace{0.1cm}
    % \State \SR{what are $\bm{\Dataset}_i^{s}$ and $\bm{\Dataset}_i^{q}$ ????}
    \For {all $\Tau_i$}
        \vspace{0.1cm}
        \State Sample $K$ data points $\bm{\Dataset}_i^{s}=\{(\textit{\textbf{x}}_j,\textit{\textbf{y}}_j)\}_{j=1}^k$ from $\Tau_i$ for the inner-level updates
        \vspace{0.1cm}
        
        \State Calculate $\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})$ with respect to $K$ samples.
        \vspace{0.1cm}
        \State Compute the task-specific parameters with gradient descent using Eqn.~\eqref{eqn:task_specific_params_rmaml}.
        \vspace{0.1cm}
    \EndFor
    \vspace{0.1cm}
    \State Sample $m$ data points $\bm{\Dataset}_i^{q}=\{(\textit{\textbf{x}}_j,\textit{\textbf{y}}_j)\}_{j=1}^m$ from $\Tau_i$ for the meta-level (outer-level) update
        \vspace{0.1cm}
    \State  Compute $\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)$ using first-order approximation method of Eqn.~\eqref{eqn:derivatives13}.
    \vspace{0.1cm}
    \State Compute $\bm{\theta}^{(t+1)}$ using Eqn.~\eqref{eqn:rmaml_1}.
    \vspace{0.1cm}
    % \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm*}

\begin{figure}[t]
\centering
\includegraphics[scale=0.25, keepaspectratio]{Figures/stiefellayer.png}
\label{fig:Stiefel-layer}
\caption{Stiefel layer Figure}
\end{figure} 


==> Sections/Related_works.tex <==
\section{Related work}
\label{Sec:Related_work}


==> Sections/Results.tex <==
\section{Experiments and Results}
\label{Sec-Results}

\subsection{Evaluation Scenarios and Datasets}
We evaluate our proposed method across different few-shot classification tasks. Following the experimental setting provided by \cite{chen2019closer,tabealhojeh2023rmaml}, we address both \emph{single-domain} and \emph{cross-domain} scenarios. In the single-domain experiments, the meta-train, meta-validation, and meta-test tasks are sampled from one dataset, while in the cross-domain scenarios, the meta-test tasks are from a different dataset. Thereby the effect of domain shift in our proposed method is studied in this scenario.

\subsubsection{Single-domain image classification}

To address the single-domain scenario, we conduct two scenarios including object recognition and fine-grained image classification. Mini-ImageNet \citep{ravi2016optimization} is used for object recognition, which includes a subset of 100 classes from the ImageNet dataset \citep{vinyals2016matching} and 600 images sampled from each class. Following the setting provided by Ravi and Larochelle \citep{ravi2016optimization}, the dataset is split into randomly selected 64, 16, and 20 classes for meta-train, meta-validation and meta-test, respectively.

For fine-grained image classification, we use the CUB-200-2011 (CUB) \citep{wah2011caltech} and FC100 \citep{krizhevsky2009learning} datasets. The CUB dataset consists of 11,788 images belonging to 200 different classes of birds. Following the evaluation protocol of \citep{hilliard2018few}, the dataset is randomly divided into the train, validation, and test meta-sets with 100, 50, and 50 classes respectively.
The FC100 dataset is based on the popular object classification dataset CIFAR100 \citep{krizhevsky2009learning} and offers a more challenging few-shot scenario, because of the lower image resolution and using more challenging meta-training/test splits that are separated according to the object superclasses. The dataset contains 100 object classes and each class has 600 samples of 32×32 color images. These 100 classes belong to 20 superclasses. Following the splits proposed by Krizhevsky et al. \citep{oreshkin2018tadam}, meta-training data contain 60 classes from 12 super-classes. Meta-validation and meta-test sets are from 20 classes belonging to 4 super-classes, respectively. Splitting the data according to the 500 super-classes minimizes the information overlap between training and validation/test tasks.

\subsubsection{Cross-domain image classification} 
    One key aspect of few-shot experiments is investigating the domain shift's effect between the meta-train and meta-test datasets on the meta-learning algorithm. For instance, one can observe that the domain gap between the meta-train and meta-test classes of miniImageNet is larger than that of CUB in a word-net hierarchy \citep{miller1995wordnet}. Thus, meta-learning on miniImageNet is more challenging than the CUB dataset. Hence, we also address the cross-domain scenario in our experimental setup. The cross-domain experiment enables us to study the effect of domain shift on our proposed method, although our method was originally developed for single-domain classification.

    Following the scenarios provided by state-of-the-art works \citep{chen2019closer}, we conduct \emph{mini-ImageNet$\rightarrow$CUB} and \emph{Omniglot$\rightarrow$EMNIST} cross-domain experiments. For the \emph{mini-ImageNet$\rightarrow$CUB} experiment, all of the $100$ classes of mini-ImageNet are used as meta-train set, while 50 meta-validation and 50 meta-test classes are sampled from CUB. For \emph{Omniglot$\rightarrow$EMNIST} experiment,
    we follow the setting proposed by Dong and Xing \citep{dong2018domain}, where the non-Latin characters of Omniglot dataset are used as the meta-train classes and the EMNIST dataset \citep{cohen2017emnist} that contains 10-digits and upper and lower case alphabets in English, is used for our meta-validation and meta-test classes. In total, the meta-train set consists of 1597 classes from the Omniglot dataset, while the 62 classes of EMNIST are split into 31 classes for meta-validation and 31 classes for meta-test sets. 


\subsection{Experimental Details}
We use the standard $N\text{-way}$ $k\text{-shot}$ classification setups, in which every task instance contains randomly sampled classifying images from $N$ different categories of the meta-train set. For each class, we sample $k$ instances as our support set and $q$ instances for the query set. For the meta-test phase, we run 600 experiments and report the average classification accuracy and the 95\% confidence interval of these 600 trials as the final result. $N$, $k$, and $q$ are sampled similarly to the meta-train stage. In our experiments, $N$ is set to 5 for all of the experiments across all datasets. %We apply standard data augmentation operations including random crop, left-right flip, and color jitter in the meta-train set, while no such data augmentation strategies are used for meta-validation and meta-test sets. For cross-domain character recognition (Omniglot$\rightarrow$EMNIST) experimental setup, the white-on-black EMNIST data are inverted to black-on-white, as in Omniglot. Moreover, since Omniglot characters are black-and-white, center-aligned and rotation sensitive, we do not use data augmentation in this experiment. 

For mini-ImageNet and CUB datasets, we use a four-layer convolutional backbone (Conv-4) with an input size of $84\times 84$. We also use the ResNet-18 backbone network with an input size of $224\times 224$, while for the Fc100 experiment, we use Conv4 and ResNet12 backbone networks. We also use Conv4 for cross-domain character recognition (\emph{Omniglot$\rightarrow$EMNIST}) experimental setup, while ResNet-18 network is used for \emph{mini-ImageNet$\rightarrow$CUB} experiment.

In all of the experiments across every network backbone, we assume that the parameters of the last fully connected layer of the network are orthonormal and lie on a Stiefel manifold. FORML meta-learns this matrix using the Riemannian operators, as described in Algorithm~\ref{alg-RMAML}. FORML optimizes the parameters of the remaining layers in Euclidean space. All the experiments were performed on a single NVIDIA V100 GPU with a memory capacity of 32GB. 

\subsubsection{Hyper-parameter setups} 
Table~\ref{tab:notations} introduces the notation used for the Steifel and Euclidean hyper-parameters. In the \textbf{single-domain} setup: 
\begin{itemize}
    \item $\alpha$ is set to $0.1$ for experiments with Conv4 backbone architecture, while it is set to $0.01$ for the others. 
    \item $\widehat\eta$ is set to $10^{-3}$ for all experiments with Conv4 backbone architecture.
    \item $\widehat\eta$ is set to $10^{-4}$ for experiments on the CUB and Mini-ImageNet datasets using ResNet-18 backbone architecture.
    \item In FC100 classification experiments, the hyper-parameters setting of Conv4 and ResNet-12 backbones are equal to those of the CUB experiments with Conv4 and ResNet-18, respectively. 
\end{itemize}

Similarly, for the experiments in the \textbf{cross-domain} setup: 
\begin{itemize}
    \item the value of $\alpha$ is set to $0.01$ for mini-ImageNet$\rightarrow$CUB, and is set to $0.05$ and $0.1$ for Omniglot$\rightarrow$EMNIST 1-shot and 5-shot experiments, respectively. 
    \item $\widehat\eta$ for mini-ImageNet$\rightarrow$CUB is set $5\times10^{-4}$, while it is set to $10^{-3}$ and $10^{-4}$ for Omniglot$\rightarrow$EMNIST 1-shot and 5-shot experiments, respectively.
\end{itemize}

For all experiments, the learning rate $\widetilde\eta$ and the weight decay $\lambda_{\widetilde\eta}$ are set to $10^{-3}$ and $0$. Similarly, the value of $\lambda_{\widehat\eta}$ is set to $0$ for experiments with Conv4 backbone architecture, while it is set to $10^{-4}$ for experiments with ResNet-18 architectures. All hyper-parameters are obtained by trial and error and for all experiments, the batch size and the number of inner-level updates for training are always set to 4 and 5, respectively.

\begin{table}[]
\centering
\caption{Notations and descriptions of hyper-parameters for experiments with RMAML.}
\label{tab:notations}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Symbol} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Learning\\ Rate\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Weight\\ Decay\end{tabular}} & \multicolumn{1}{c|}{Parameters} & \multicolumn{1}{c|}{Loop} \\ \hline
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\ \hline
$\alpha$ & $\checkmark$ & $\times$ & \multirow{2}{*}{Stiefel} & \multirow{2}{*}{Inner}  \\
$\lambda_{\alpha}$ & $\times$ & $\checkmark$ &  &  \\ \hline
$\widetilde\eta$ & $\checkmark$ & $\times$ & \multirow{2}{*}{Stiefel} & \multirow{2}{*}{Outer}  \\
$\lambda_{\widetilde\eta}$ & $\times$ & $\checkmark$ &  &  \\ \hline

$\widehat\eta$ & $\checkmark$ & $\times$ & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non\\ Stiefel\end{tabular}} & \multirow{2}{*}{Outer}  \\
$\lambda_{\widehat\eta}$ & $\times$ & $\checkmark$ &  &  \\ \hline

\end{tabular}
\end{table}
% \end{description}

% In the experiments mentioned above, the value of weight decay for the 
\subsubsection{Methods used for comparison}
In all our experiments, we compare RMAML with the following methods as briefly discussed below.
\begin{description}
    \item [\textbf{Baseline}] is the standard procedure of transfer learning, in which a network is learned and then fine-tuned by fixing the pre-trained feature extractor (convolutional) layers and fine-tuning the last fully-connected layer using the support set. The standard cross-entropy loss is used to optimize the learnable parameters of the network.
    % \item [\textbf{MatchingNet}] \citep{vinyals2016matching} is a metric-learning based meta-learning approach that classifies the query set based on the similarity between the query-support sets, after embedding them into a shared feature space.
    % \item [\textbf{ProtoNet}] \citep{snell2017prototypical} is another metric-based meta-learning method that aims to reduce the effect of outliers by comparing the similarity of the query with the class prototypes (\textit{i.e.} class centroids) of the support set.
    % \item [\textbf{RelationNet}] \citep{sung2018learning} can be regarded as an extension of MatchingNet in which the learned metric is defined by a neural network. 
    \item [\textbf{MAML}] \citep{finn2017model} is an optimization-based meta-learning method discussed in Section~\ref{subsec:MAML}.
\end{description}
We directly used the results reported in \citep{chen2019closer} for the above described methods in Tables~\ref{tab1: all experiments} and~\ref{tab:cross-exp} for comparison against RMAML.
\subsection{Results for Single-Domain Experiments}

We conduct the standard 5-way 1-shot and 5-shot experiments for single-domain few-shot classification. Table~\ref{tab1: all experiments} presents few-shot classification results for single-domain experiments with different backbone networks, on mini-ImageNet and CUB datasets. Among all the experimental setups, RMAML has a significant improvement over its non-Riemannian counterpart (\textit{i.e} MAML) in terms of classification accuracy (\textit{e.g.} $75.79\pm0.92$ vs $68.42\pm1.07$ for the 1-shot experiment on the CUB dataset using ResNet18 backbone). Moreover, as the depth of the backbone network is increased (Conv4 $\rightarrow$ ResNet18), RMAML either outperforms or achieves comparable results with respect to the other meta-learning methods considered for comparison for both 1-shot and 5-shot experiments.
We also adopt Conv4 and ResNet12 backbones to assess our algorithm against FC100 dataset. As shown in Table~\ref{tab:FC100-exp}, we observe that RMAML improves the few-shot recognition performance on FC100 dataset, compared to its Euclidean counterpart and other methods. 

Compared to its Euclidean counterpart, as it is evident in Tables~\ref{tab1: all experiments} and \ref{tab:FC100-exp}, our proposed algorithm RMAML has remarkably outperformed MAML across all the backbone network architectures for all the single domain experimental setups. A pictorial comparison between RMAML and MAML is shown in Fig.~\ref{fig:MAML vs RMAML} for better understanding. Furthermore, as the depth of the backbone network is increased, MAML fails to improve its results on the CUB dataset due to over-fitting to its training set, while no such over-fitting is observed for RMAML and its performance continues to improve as the networks become deeper. Moreover, one can clearly observe that for experiments on miniImageNet, RMAML outperforms MAML by a significant margin as the depth of the network increases; even though both these methods overfit to the training set for the ResNet-18 backbone.

\begin{table}
\centering
\caption{Few-shot classification accuracies for mini-ImageNet and CUB datasets against different backbone networks are shown in the last 4 columns. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab1: all experiments}
\begin{tabular}{llll}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|c|l|cccc|}%@{\extracolsep{\fill}}}
\hline%toprule
\multicolumn{1}{c}{\textbf{Dataset}}  & \textbf{Method} & \textbf{Conv-4} & \textbf{ResNet-18} \\ \hline
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 1-shot\end{tabular}} &  MAML \cite{chen2019closer}  & $54.73\pm0.97$ & $68.42\pm1.07$\\
& FORML (ours) & $\bm{58.86\pm0.99}$ & $\bm{71.68\pm0.99}$\\
 \hline%midrule
 \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 5-shot\end{tabular}} & MAML \cite{chen2019closer} & $75.75\pm0.76$& $83.47\pm0.62$\\
 & FORML (ours) & $\bm{77.93\pm0.95}$& \bm{$84.76 \pm 0.64$} \\
 \hline%midrule
 \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 1-shot\end{tabular}} 
 &MAML \cite{chen2019closer} &$46.47\pm0.82$ & $49.61\pm0.92$\\
 % & Reptile \cite{nichol2018first} & $47.07\pm0.26$ &  $-$& $-$ & $-$\\
& FORML (ours) &\bm{$47.89\pm0.80$} & \bm{$51.23 \pm 0.89$}\\
 \hline%midrule
 \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 5-shot\end{tabular}} 
 & MAML \cite{chen2019closer} &$62.71\pm0.71$ &$65.72\pm0.77$\\
 % & Reptile \cite{nichol2018first}  & $62.74\pm0.38$ &  $-$& $-$ & $-$\\
& FORML (ours) & \bm{$64.46\pm0.68$} & \bm{$67.89\pm0.75$} \\
 \bottomrule
\end{tabular}
\end{table}


% \begin{table}
% \centering
% \caption{Few-shot classification accuracies for mini-ImageNet and CUB datasets against different backbone networks are shown in the last 4 columns. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab1: all experiments}
% \begin{tabular}{llllll}
% % \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|c|l|cccc|}%@{\extracolsep{\fill}}}
% \hline%toprule
% \multicolumn{1}{c}{\textbf{Dataset}}  & \textbf{Method} & \textbf{Conv-4} & \textbf{Conv-6} & \textbf{ResNet-10} & \textbf{ResNet-18} \\ \hline
% \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 1-shot\end{tabular}} &  MAML \cite{chen2019closer}  & $54.73\pm0.97$ &  $66.26\pm1.05$& $70.32\pm0.99$ & $68.42\pm1.07$\\
% & FORML (ours) & $\bm{58.86\pm0.99}$ & $\bm{67.29\pm0.99}$ & $\bm{70.96\pm0.97}$ & $\bm{71.68\pm0.99}$\\
%  \hline%midrule
%  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 5-shot\end{tabular}} & MAML \cite{chen2019closer} & $75.75\pm0.76$& $78.82\pm0.70$& $80.93\pm0.71$ & $83.47\pm0.62$\\
%  & FORML (ours) & $\bm{77.93\pm0.95}$& $\bm{79.76\pm0.98}$7 & \bm{$82.45 \pm 0.69$}  & \bm{$84.76 \pm 0.64$} \\
%  \hline%midrule
%  \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 1-shot\end{tabular}} 
%  &MAML \cite{chen2019closer} &$46.47\pm0.82$ &$50.96\pm0.92$& $54.69\pm0.89$& $49.61\pm0.92$\\
%  % & Reptile \cite{nichol2018first} & $47.07\pm0.26$ &  $-$& $-$ & $-$\\
% & FORML (ours) &\bm{$47.89\pm0.80$} & \bm{$51.68\pm0.55$}& \bm{$55.13 \pm 0.88$} & \bm{$51.23 \pm 0.89$}\\
%  \hline%midrule
%  \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 5-shot\end{tabular}} 
%  & MAML \cite{chen2019closer} &$62.71\pm0.71$& $66.09\pm0.71$ &$66.62\pm0.83$ &$65.72\pm0.77$\\
%  % & Reptile \cite{nichol2018first}  & $62.74\pm0.38$ &  $-$& $-$ & $-$\\
% & FORML (ours) & \bm{$64.46\pm0.68$} & \bm{$68.12\pm0.88$}& \bm{$68.82\pm0.85$} & \bm{$67.89\pm0.75$} \\
%  \bottomrule
% \end{tabular}
% \end{table}


\begin{table}
\centering
\caption{Few-shot classification accuracies for FC100 dataset. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab:FC100-exp}
\begin{tabular}{lllll}
\toprule
\textbf{Backbone Networks} & \multicolumn{2}{c}{\textbf{Conv4}} & \multicolumn{2}{c}{\textbf{ResNet12}} \\ 
\cmidrule(r){1-5}
\textbf{Method} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
\cmidrule(r){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-5}
Baseline & $32.48\pm 0.58$ & $47.15 \pm 0.67$ & $38.24 \pm 0.63$ & $56.87 \pm 0.71$ \\
% MatchingNet & $35.36 \pm 0.68$ & $48.36 \pm 0.71$ & $40.85 \pm 0.75$ & $55.70 \pm 0.71$ \\
% ProtoNet &  $34.86 \pm 0.72$ & $48.79 \pm 0.70$ & $40.90\pm 0.73$ & \bm{$57.95\pm 0.70$}\\
% RelationNet & $37.52\pm 0.74$ & $48.94\pm 0.72$ & $37.02\pm 0.79$ & $49.83\pm 0.73$ \\
MAML\cite{chen2019closer} & $36.70\pm 0.83$ & $47.69\pm0.79$ & $40.15\pm0.78$ & $54.13\pm0.77$ \\
FORML (ours) & \bm{$38.82\pm0.72$} & \bm{$49.05\pm0.88$} & \bm{$41.30\pm0.68$} & \bm{$57.35\pm0.84$}  \\ 
\bottomrule

\end{tabular}
\end{table}

\subsection{Results for Cross-Domain Experiments}
Table~\ref{tab:cross-exp} shows the results of mini-ImageNet$\rightarrow$CUB and Omniglot$\rightarrow$EMNIST experiments. For 1-shot Omniglot$\rightarrow$EMNIST experiment, RMAML  outperforms all other methods (except the RelationNet method) as shown in Table~\ref{tab:cross-exp}, while still obtaining comparable results to MatchingNet and RelationNet for the 5-shot experiment. Moreover, RMAML has remarkably outperformed MAML by more than $9\%$, in terms of classification accuracy in mini-ImageNet$\rightarrow$CUB experiment.  However, in this experiment one can observe that the Baseline method outperforms all the other methods (including MAML and RMAML) as it is much simpler to adapt to the target domain by learning a new parameterized classifier layer for the Baseline method. On the other hand, meta-learning methods fail to overcome the diverse and significant domain gap between the meta-train and meta-test sets in comparison to Baseline method~\citep{vinyals2016matching, chen2019closer}. Having said that, RMAML still obtains competitive results in terms of classification accuracy against other meta-learning methods. Excluding the Baseline results, RMAML obtains the second best result in 1-shot Omniglot$\rightarrow$EMNIST and 5-shot mini-ImageNet$\rightarrow$CUB  experiments and the third stage in 1-shot Omniglot$\rightarrow$EMNIST experiment. Compared to MAML, our proposed method can achieve results analogous to its Euclidean counterpart, while it can strongly outperforms MAML when deeper backbone network is used. For instance, unlike MAML, RMAML prevents ResNet18 from over-fitting in mini-ImageNet$\rightarrow$CUB experiment. 



\begin{table}
\centering
\caption{Classification accuracies for \textbf{Omniglot$\rightarrow$EMNIST} and \textbf{mini-ImageNet$\rightarrow$CUB} cross-domain experimental setup.}\label{tab:cross-exp}
\begin{tabular}{llll}
\toprule
 & \multicolumn{2}{l}{\textbf{Omniglot$\rightarrow$EMNIST}} & \textbf{mini-ImageNet$\rightarrow$CUB} \\ 
 \cmidrule(r){2-4}
\textbf{Backbone Networks} & \multicolumn{2}{l}{\textbf{Conv4}} & \multicolumn{1}{l}{\textbf{ResNet18}} \\ 
\midrule

\textbf{Method} & \textbf{1-shot} & \textbf{5-shot} & \textbf{5-shot} \\ \cmidrule(r){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-4}
Baseline & $63.94\pm0.87$ & $86.00\pm0.59$ & \bm{$65.57\pm0.70$} \\
% MatchingNet & $72.71\pm0.79$ & $87.60\pm0.56$ & $53.07\pm0.74$ \\
% ProtoNet &  $70.43\pm0.80$ & $87.04\pm0.55$ & $62.02\pm0.70$ \\
% RelationNet & \bm{$75.55\pm0.87$} & \bm{$88.94\pm0.54$} & $57.71\pm0.73$ \\
MAML & $72.04\pm 0.83$ & \bm{$88.24\pm0.56$}  & $51.34\pm0.72$ \\
FORML (ours) & \bm{$72.78\pm 0.82$} & $87.41 \pm0.57 $  &  $56.43\pm0.71$ \\ \bottomrule
\end{tabular}
\end{table}




\subsection{Computational Complexity}\label{subsec:computational-complexity}



==> Sections/Sections/Abstract.tex <==
\begin{abstract}
  Many methods formulate the Meta-learning problem as a bi-level optimization in which the task-specific and the meta-parameters are updated in the inner and outer loops of optimization, respectively. However, performing the optimization in the Riemannian space, where the parameters and meta-parameters are located on Riemannian manifolds is computationally intensive. Unlike the Euclidean methods, backpropagation needs computing the second-order derivatives that include backward computations through the Riemannian operators such as retraction and orthogonal projection. In this paper, we introduce a Hessian-free approach that uses a first-order approximation of derivatives.          
\end{abstract}

==> Sections/Sections/Conclusion.tex <==
\label{Sec-Conclusion}

==> Sections/Sections/Introduction.tex <==
\section{Introduction}
\label{Sec-Introduction}
\IEEEPARstart{M}{eta-learning} has attracted growing attention recently, owing to its capability to learn from several tasks and generalize to unseen ones. From the Optimization-based point of view, meta-learning can be formulated as a bi-level optimization problem, consisting of two optimization levels. At the outer level, a meta-learner extracts the meta-knowledge (the \textit{how to learn } knowledge) from specific tasks, whereas at the inner level, each specific task is learned via a base-learner. Among different approaches to meta-learning, in optimization-based methods (please refer to ) the meta-learner \textit{learn how to optimize} the task-specific base learners. In other words, both the meta and base learners are (usually gradient descent) optimizers. Then the meta-knowledge can be considered as the step-size, gradient, or anything that can affect or improve the inner-level optimizers. 

In practice, numerous learning tasks are modeled as optimization problems with nonlinear constraints. For instance, many classic machine learning problems such as Principal component analysis (PCA) \cite{yuan2019online}, independent component analysis (ICA) \cite{hyvarinen2000independent} and subspace learning \cite{chakraborty2020intrinsic} are cast as optimization problems with orthogonality constraints. Also, modern deep neural networks benefit from applying the orthogonality constraint on their parameter matrices, which results in significant advantages such as increasing the accuracy and attaining a faster convergence rate \citep{bansal2018can}, improving the generalization \citep{cogswell2015reducing} and stabilizing the distribution of neural activations during the training of Convolutional Neural Networks (CNNs) \citep{huang2018building}. A popular way to incorporate nonlinear constraints into optimization frameworks is to make use of Riemannian geometry and formulate constrained problems as optimization on Riemannian manifolds \cite{lin2008riemannian}. In this case, Euclidean meta-learning with nonlinear constraints is cast as meta-learning on Riemannian manifolds, namely learning to optimize in Riemannian spaces. To do so, the optimization algorithm should be respectful to the Riemannian geometry, which can be achieved by utilizing the Riemannian operations such as \textit{retraction, orthogonal projection} and \textit{parallel transport}. However,  learning optimizers on Riemannian manifolds need second-order differentiation through the nonlinear Riemannian optimization, which is complex and computationally expensive.

In this paper, we propose a Riemannian meta-optimization method that uses a first-order approximation to calculate the derivatives. In the inner loop of our algorithm, base learners are optimized using a limited number of steps on the Riemannian manifold. At the outer loop, to update the meta-optimizer, instead of computing the derivatives through the entire inner-level path, they are computed by only considering the last step of the inner-level optimization. In this way, learning the meta-optimizer does not need to differentiate through the complex Riemannian optimization in the inner loop. Therefore, our method avoids the exploding gradient issue caused by computing products of Hessian and gradients of the retraction, resulting in computational efficiency and stability of the bi-level optimization. We empirically show that our proposed method can be trained efficiently and learn a good optimization trajectory compared to other methods.

The rest of the paper is organized as follows. Section~\ref{Sec-Preliminaries} covers the common foundations on which we will base our proposed algorithms. Section~\ref{Sec-method} describes our proposed technique,~\textit{i.e} First Order Riemannian Meta-Learning (FORML) methods. The experimental analysis, evaluations, and results are presented in Section~\ref{Sec-Results}. Finally, Section~\ref{Sec-Conclusion} concludes the paper.


==> Sections/Sections/Method.tex <==
\section{Proposed Method}
\label{Sec-method}
Generally, the optimization-based meta-training (learn to optimize) on Riemannian manifolds can be formulated as \cite{tabealhojeh2023rmaml}:
\begin{align}
     \label{Eq:general-Riemannian-meta-train}
\bm{\theta}_{meta}^*= \underbrace{\min_{\bm{\theta}\in\Manifold}{\frac{1}{N} \sum_{i=1}^{N}{\Loss_{i}\big(\bm{\Dataset}_i^{q},\overbrace{\bm{\phi}_{i}^{*}}^{\text{inner-level}})}}}_{\text{outer-level}}\big) 
\end{align}

where $N$ is the number of training tasks, $\bm{\theta}$ and $\bm{\phi}$ respectively indicate the meta-parameters and parameters of the meta-learner that are located on a Riemannian manifold $\Manifold$, ~\textit{i.e} $\bm{\theta}, \bm{\phi}\in\Manifold$. $\Loss_i$ is the loss function of the $i^{th}$ task, whereas $\Dataset_i=\{\bm{\Dataset}_i^{s},\bm{\Dataset}_i^{q}\}$ demonstrates the meta-train dataset of $i^{th}$ task. The support set $\bm{\Dataset}_i^{s}$ and the query set $\bm{\Dataset}_i^{q}$ are respectively analogous to training and validation datasets in classic supervised training. Eqn.~\eqref{Eq:general-Riemannian-meta-train} demonstrate two levels of optimization. The outer loop (or the meta-optimizer) learns the optimal meta-parameter, ~\textit{i.e} $\bm{\theta}_{meta}^*$ using query datasets from a distribution of $N$ training tasks and the optimal task-specific parameters $\bm{\phi}_{i}^*$. However, as the $\bm{\phi}_{i}^*$ is unknown, it can be solved as another optimization problem (the inner-level optimization). Therefore, Eqn.~\eqref{Eq:general-Riemannian-meta-train} can be considered as a bilevel optimization; a constrained optimization in which each constraint is itself an optimization problem:
\begin{align}
    \label{Eq:bi-level-Riemannian}
    \begin{split}
\bm{\theta}_{meta}^*=\min_{\bm{\theta}\in\Manifold}{\frac{1}{N} \sum_{i=1}^{N}{\Loss_{i}\big(\bm{\Dataset}_i^{q},\bm{\phi}_i^*\big)}}
 \\ 
 \text{subject to}~~\bm{\phi}_i^*=\gfun(\bm{\Dataset}_i^{s},\bm{\theta}_{meta}^*)
\end{split}
\end{align}

Where $\gfun(\bm{\Dataset}_i^{s},\bm{\theta}_{meta}^*)$ is (usually) a gradient descent optimizer which is dependent on the meta-knowledge, $\bm{\theta}_{meta}^*$. The meta-knowledge can be interpreted as learning an appropriate parameter initialization \cite{tabealhojeh2023rmaml} or even learning to optimize a LSTM model \cite{gao2020learning,gao2022learning}. Assuming the meta-parameter as an initial point, the bilevel optimization problem of qn.~\eqref{Eq:bi-level-Riemannian}, can be solved by performing two nested loops. At the inner loop, a limited number of gradient descent steps are performed to optimize each task-specific parameter $\bm{\phi}_i^*$ using the meta-parameter as an initial point,~\textit{i.e} $\bm{\phi}_i^{(0)}=\bm{\theta}_{meta}$, and the outer loop performs a gradient descent update for the meta-parameter, $\bm{\theta}_{meta}$.  Each step of the inner loop optimization problem can be formulated as follows: 

\begin{equation}
\begin{aligned}
\label{eqn:task_specific_params_rmaml}
\bm{\phi}_i^{(l+1)}=
R_{\bm{\phi}_i^{(l)}}\left(-\alpha \pi_{\bm{\phi}_i^{(l)}}\big(\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})\big)\right), l\ge 1
\end{aligned}    
\end{equation}
in which the Euclidean gradient vector $\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})$ is projected to the tangent space of $\bm{\phi}_i^{(l)}$ and then the parameters are updated by performing the \textit{retraction} operator {$R_{\bm{\phi}_i^{(l)}}$}.

Moreover, a single step of gradient decent in Riemannian space for the outer loop is as follows:
%\begin{equation}
%\begin{aligned}
%\label{eqn:rmaml_2}
%\bm{\theta}^{(t+1)}=\\
%R_{\bm{\theta}^{(t)}}\left(-\beta \left( \sum_{\Tau_i \in \Tau}\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}^{(t)}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)\right)\right)  
%\end{aligned}    
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\label{eqn:rmaml_2}
%\bm{\theta}_{meta}^*=\\
%R_{\bm{\theta}}\left(-\beta \left( \sum_{\Tau_i \in \Tau}\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)\right)\right)  
%\end{aligned}    
%end{equation}
%\HT{where for each task, the projected gradient vector is parallely transported from the tangent space of $\bm{\phi}_i$ (\textit{i.e.} $\bm{\phi}_i^{(k)}$ using $k$ inner-level updates) to the tangent space of the current meta-parameter $\bm{\theta}^{(t)}$. Thus, the meta-parameter is updated by performing the \textit{retraction} operator $R_{\bm{\theta}^{(t)}}$. Equivalently Eqn.~\eqref{eqn:rmaml_2} can be written as follows}:
%\begin{align}
%\label{eqn:rmaml_1}
%\bm{\theta}_{meta}^*= R_{\bm{\theta}}\left(-\beta \sum_{\Tau_i \in \Tau}{\pi_{\bm{\theta}}}\Big(\nabla_{\bm{\theta}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)\right)     
%\end{align}
\begin{align}
\label{eqn:rmaml_1}
\bm{\theta}^{(t+1)}= R_{\bm{\theta}^{(t)}}\left(-\beta \sum_{i=1}^{M}{\pi_{\bm{\theta}^{(t)}}}\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)\right)     
\end{align}
where to calculate $\bm{\theta}^{(t+1)}$, the Euclidean gradient vector of each task, $\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$ is orthogonally projected to the tangent space of the current meta-parameter by $\pi_{\bm{\theta}^{(t)}}(.)$ operation. Then the summation over the Riemannian gradient of all the tasks is retracted to the manifold. To compute the gradient vector $\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$
For each task, differentiating through the inner-level optimization path is needed. In other words, calculating $\pi_{\bm{\theta}^{(t)}}\Big(\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$ requires a gradient of the gradients and needs a heavy computation for the second-order derivatives that include backward computations through the Riemannian operators such as retraction and orthogonal projection. Assuming that $k$ Riemannian gradient descent steps are performed in the inner level optimization, then: 

\begin{align}
\label{eqn:nabla_derivatives}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)= \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)     
\end{align}

where $\bm{\phi}_i^{(k)}$ is the result of inner-level optimization chain:
\begin{multline}
\label{eqn:inner_chain}
\bm{\phi}_i^{(k)}=
R_{\bm{\phi}_i^{(k-1)}}\left(-\alpha \pi_{\bm{\phi}_i^{(k-1)}}\left(\nabla_{\bm{\phi}_i^{(k-1)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(k-1)})\right)\right)  \\  
\bm{\phi}_i^{(k-1)}=
R_{\bm{\phi}_i^{(k-2)}}\left(-\alpha \pi_{\bm{\phi}_i^{(k-2)}}\left(\nabla_{\bm{\phi}_i^{(k-2)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(k-2)})\right)\right)    \\    
\vdots \\
\bm{\phi}_i^{(0)}=\bm{\theta}^{(t)}  
\end{multline}    


Using the chain rule, the derivative in the~\eqref{eqn:nabla_derivatives} becomes as follows:

\begin{align}
\label{eqn:nabla_derivation_unfolded1}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
= \frac{\partial \Loss_i}{\partial \bm{\phi}_i^{(k)}}\frac{\partial \bm{\phi}_i^{(k)}}{\partial \bm{\theta}^{(t)}}
\end{align}

Considering the inner-level chain of the~\eqref{eqn:nabla_derivation_unfolded1}, the $\frac{\partial \bm{\phi}_i^{(k)}}{\partial \bm{\theta}^{(t)}}$ term can be further unfolded as follows:

\begin{multline}
\label{eqn:nabla_derivation_unfolded2}
\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
= \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)}{\partial \bm{\phi}_i^{(k)}} \prod_{l=1}^{k}{  \frac{\partial \bm{\phi}_i^{(l)}}{\partial \bm{\phi}_{i}^{(l-1)}}}\\
= \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)}{\partial \bm{\phi}_i^{(k)}}\\
\prod_{l=1}^{k}{\frac{\partial \bigg( R_{\bm{\phi}_i^{(l-1)}}\left(-\alpha \pi_{\bm{\phi}_i^{(l-1)}}\left(\nabla_{\bm{\phi}_i^{(l-1)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l-1)})\right)\right)\bigg)}{\partial \bm{\phi}_{i}^{(l-1)}}}
\end{multline}

The equation contains the second-order differentiation terms that pass through the Riemannian operations of the inner-level optimization steps, which require heavy calculation and computational resources. 

In the next section, we formulate a first-order approximation for the~\eqref{eqn:nabla_derivation_unfolded2}, that enables us to perform a hessian-free bi-level optimization for the Riemannian meta-learning problem. 

\subsection{First Order approximation: From Euclidean space to Stiefel manifold}
without loss of generality, let us consider exactly one update at the inner-level chain of~\eqref{eqn:nabla_derivation_unfolded2}. Thus this step of inner-level optimization is as follows:

\begin{align}
\label{eqn:inner_single_step}
    \bm{\phi}_i^{(1)}=
R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}_i^{(t)})\right)\right)
\end{align}

Therefore, the equation \eqref{eqn:nabla_derivation_unfolded2} will be changed as follows:
\begin{multline}
    \label{eqn:nabla_derivatives_single}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)=\\
    \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}} \frac{\partial \bigg( R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)}{\partial \bm{\theta}^{(t)}}
\end{multline}

The above expression is general for Riemannian manifolds. For instance, using the Euclidian operations on the Euclidean manifold, one can write the equation~\eqref{eqn:nabla_derivatives_single} as:
\begin{multline}
    \label{eqn:nabla_derivatives_single_Euc}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)=\\
    \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}} 
    \frac{\partial \bigg( \bm{\theta}^{(t)}-\alpha (\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\bigg)}{\partial \bm{\theta}^{(t)}}
\end{multline}

which can be further simplified as:

\begin{multline}
\label{eqn:nabla_derivatives_single_Euc_sim}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)=\\
    \frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}  \bigg( \bm{I}-\alpha (\nabla^{2}_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\bigg)
\end{multline}

For the Euclidean spaces, the first-order approximation of~\eqref{eqn:nabla_derivatives_single_Euc_sim}, FOMAML [] can be calculated by ignoring the second-order derivatives of~\eqref{eqn:derivatives9}:
\begin{align}
    \label{eqn:derivatives9}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    =\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}
\end{align}

  On the other hand, calculating such an approximation for the Riemannian spaces is not straightforward. In the rest of the section, we derive the formulation of first-order approximation on Stiefel manifolds. To do so, we compute the $\frac{\partial \bigg( R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)}{\partial \bm{\theta}^{(t)}}$ term of~\eqref{eqn:nabla_derivatives_single} as follows. For simplification, we indicate the $\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})$ as $\nabla_{\bm{\theta}^{(t)}}\Loss_i$, and $d$ indicates the derivative with respect to $\bm{\theta}^{(t)}$, \textit{i.e.} $\frac{\partial(\cdot)}{\partial \bm{\theta}^{(t)}}$:

\begin{gather*}
    d\bigg(R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i\right)\right)\bigg)=\\
    d\bigg( \bm{\theta}^{(t)}-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i\right) \bigg)=
    \\d(\bm{\theta}^{(t)})-d\bigg(\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i\right) \bigg)=
    d(\bm{\theta}^{(t)})-\\\alpha d\bigg( \nabla_{\bm{\theta}^{(t)}}\Loss_i-\bm{\theta}^{(t)}\frac{(\bm{\theta}^{(t)})^{T} \nabla_{\bm{\theta}^{(t)}}\Loss_i-(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)}}{2} \bigg)=\\
    d(\bm{\theta}^{(t)})-\alpha d(\nabla_{\bm{\theta}^{(t)}}\Loss_i)+0.5\alpha d\bigg( \bm{\theta}^{(t)} (\bm{\theta}^{(t)})^{T} \nabla_{\bm{\theta}^{(t)}}\Loss_i\bigg)\\-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)} \bigg)=
    d(\bm{\theta}^{(t)})-\alpha d(\nabla_{\bm{\theta}^{(t)}})\\+0.5\alpha d\bigg( \nabla_{\bm{\theta}^{(t)}}\bigg)-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)} \bigg)=\\
    d(\bm{\theta}^{(t)})-0.5\alpha d(\nabla_{\bm{\theta}^{(t)}})-0.5\alpha d\bigg(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)} \bigg)=\\
    d(\bm{\theta}^{(t)})-0.5\alpha d(\nabla_{\bm{\theta}^{(t)}}\Loss_i)
    -0.5\alpha d(\bm{\theta}^{(t)})(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)}\\-0.5\alpha \bm{\theta}^{(t)}d(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)}-0.5\alpha \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}d(\bm{\theta}^{(t)})
\end{gather*}
The second and fourth terms of the above formula contain second-order derivatives.By ignoring those terms and using $\vect(\cdot)$ operator, the derivatives with respect to $\bm{\theta}$ which is an orthogonal matrix (a point on Stiefel manifold) can be written as:
\begin{gather*}
 \label{eqn:derivatives11}
  \bm{I}\vect( d(\bm{\theta}^{(t)})-0.5\alpha \vect( d(\bm{\theta}^{(t)})(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}\bm{\theta}^{(t)})\\-0.5\alpha \vect(\bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T}d(\bm{\theta}^{(t)}))=\\
  \bm{I}\vect( d(\bm{\theta}^{(t)})-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}}\Loss_i\otimes \bm{I}\bigg) \vect( d(\bm{\theta}^{(t)})\\
  -0.5\alpha\bigg(\bm{I}\otimes \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T} \bigg) \vect( d(\bm{\theta}^{(t)})=\\
\bigg(\bm{I}-0.5\alpha\big((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}}\Loss_i\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T} \big)\bigg)\vect( d(\bm{\theta}^{(t)})
\end{gather*}

Thus we will have:
\begin{multline}
    \label{eqn:derivatives12}
    \vect\bigg(d\bigg(R_{\bm{\theta}^{(t)}}\left(-\alpha \pi_{\bm{\theta}^{(t)}}\left(\nabla_{\bm{\theta}^{(t)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\theta}^{(t)})\right)\right)\bigg)\bigg)\approx \\
    \bm{I}-0.5\alpha\bigg((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}}\Loss_i\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_i)^{T} \bigg)\big(\vect( d(\bm{\theta}^{(t)})\big)
\end{multline}
Thus, the first-order approximation of~\eqref{eqn:nabla_derivatives_single} is as follows:

\begin{multline}   
    \label{eqn:final_FORML}
    \nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)
    \approx\frac{\partial \Loss_{i}\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(1)}\right)}{\partial \bm{\phi}_i^{(1)}}\\
    \bigg(\bm{I}-0.5\alpha\big((\bm{\theta}^{(t)})^{T}\nabla_{\bm{\theta}^{(t)}}\Loss_{i}\oplus \bm{\theta}^{(t)}(\nabla_{\bm{\theta}^{(t)}}\Loss_{i})^{T} \big) \bigg)
\end{multline}

%\begin{align}
%\label{eqn:rmaml_new}
%\bm{\theta}^{(t+1)}= R_{\bm{\theta}^{(t)}}\left(-\beta \sum_{i=1}^{M}%{\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right)}\right)    %
%\end{align}

 %where $\pi_{\bm{\theta}} \Big(\nabla_{\bm{\theta}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\Big)$=$\Gamma_{\bm{\phi}_i \rightarrow \bm{\theta}}\left({\pi_{\bm{\phi}_{i}}}\left(\nabla_{\bm{\phi}_i} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i\right)\right)\right) $

\begin{figure}[t]
\centering
\includegraphics[scale=0.25, keepaspectratio]{Figures/stiefellayer.png}
\caption{A sample representation of the Stiefel fully connected layer for 2D output space, where $\bm{W}=[\bm{w}_1,\bm{w}_2]$ represent the orthogonal weight matrix (lies on Stiefel manifold) and $\bm{x}$ is the input vector of the Stiefel fully connected layer. For this example, the equation~(\ref{eqn:Stiefel-layer}) will be as: $\bm{W}^{T}\bm{x}=\bm{\gamma}=[\gamma_1,\gamma_2]$.}
\label{fig:Stiefellayer}
\end{figure} 

\subsection{The proposed bi-level algorithm}
The full proposed method is outlined in Algorithm~\ref{alg-RMAML}. Practically we meta-optimize the last fully-connected layer of the backbone network using FORML on Stiefel manifold, while the other parameters are optimized on Euclidean space. Moreover, we normalize the input of the Stiefel layer. As a result, the forward computation of that fully-connected layer acts as a Cosine distance between the input vector $\textbf{x}$ and the weight vectors of the classes that are columns of the weight matrix $\textbf{W}$. (As shown in Figure~\ref{fig:Stiefellayer}).  
\begin{align}
    \label{eqn:Stiefel-layer}
    \textbf{W}^{T}\textbf{x}=\frac{\textbf{W}^{T}\textbf{x}}{\| \textbf{W} \| \| \textbf{x} \|}=\bm{\gamma}
\end{align}

\begin{algorithm*}
\centering
\caption{RMAML}\label{alg-RMAML}
\begin{algorithmic}[1]
\Require %Distribution over meta-training tasks $p(\Tau)$, inner-level learning rate $\alpha$, outer-level learning rate $\beta$.

$p(\Tau)$ denotes the distribution over meta-training tasks.

~~~$\alpha$ denotes the inner-level learning rate.

~~~$\beta$ represents the outer-level learning rate.
\vspace{0.1cm}
%\Require Inner-level learning rate $\alpha$, outer-level learning rate $\beta$.
\vspace{0.1cm}
\State Randomly initialize  $\bm{\theta}^{(0)}$
\vspace{0.1cm}
% \State \SR{What about $\bm{\theta}$ and not $\bm{\theta}_{meta}$??}
\While{not done}
    \vspace{0.1cm}
    \State Sample batch $\{\Tau_i\}_{i=1}^B$ 
    \vspace{0.1cm}
    % \State \SR{what are $\bm{\Dataset}_i^{s}$ and $\bm{\Dataset}_i^{q}$ ????}
    \For {all $\Tau_i$}
        \vspace{0.1cm}
        \State Sample $K$ data points $\bm{\Dataset}_i^{s}=\{(\textit{\textbf{x}}_j,\textit{\textbf{y}}_j)\}_{j=1}^k$ from $\Tau_i$ for the inner-level updates
        \vspace{0.1cm}
        
        \State Calculate $\nabla_{\bm{\phi}_i^{(l)}} \Loss_i(\bm{\Dataset}_i^{s},\bm{\phi}_i^{(l)})$ with respect to $K$ samples.
        \vspace{0.1cm}
        \State Compute the task-specific parameters with gradient descent using Eqn.~\eqref{eqn:task_specific_params_rmaml}.
        \vspace{0.1cm}
    \EndFor
    \vspace{0.1cm}
    \State Sample $m$ data points $\bm{\Dataset}_i^{q}=\{(\textit{\textbf{x}}_j,\textit{\textbf{y}}_j)\}_{j=1}^m$ from $\Tau_i$ for the meta-level (outer-level) update
        \vspace{0.1cm}
    \State  Compute $\nabla_{\bm{\theta}^{(t)}} \Loss_i\left(\bm{\Dataset}_i^{q},\bm{\phi}_i^{(k)}\right)$ using first-order approximation method of Eqn.~\eqref{eqn:final_FORML}.
    \vspace{0.1cm}
    \State Compute $\bm{\theta}^{(t+1)}$ using Eqn.~\eqref{eqn:rmaml_1}.
    \vspace{0.1cm}
    % \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm*}



==> Sections/Sections/Preliminaries.tex <==
\section{Preliminaries}
\label{Sec-Preliminaries}

\subsection{Riemannian manifolds}
In this section, we introduce the definition of smooth Riemannian manifolds and the required mathematical operations for applying Gradient Descent (GD) or GD-based optimization algorithms in Riemannian spaces.    
\begin{definition}[Smooth Riemannian manifold]
A smooth Riemannian manifold $\Manifold$ is a locally Euclidean space and can be understood as a generalization of the notion of a surface to higher dimensional spaces \cite{lin2008riemannian}. For each point $\textit{\textbf{P}}\in \Manifold$, the tangent space is denoted by $T_\textit{\textbf{P}}\Manifold$. The tangent space at a point $\textit{\textbf{P}}\in \Manifold$ is a vector space that consists of all vectors that are tangent to $\Manifold$ at $\textit{\textbf{P}}$.
\end{definition}
\begin{definition}[Stiefel manifold]
The Stiefel manifold $St(n,p), n \geq p$, is a Riemannian manifold that is composed of all $n \times p$ orthonormal matrices, i.e. $\{\textbf{P}\in \mathbb{R}^{n \times p}:\textbf{P}^T\textbf{P}=\textbf{I}\}$. 
\end{definition}

\begin{definition}[Manifold optimization]
Manifold optimization refers to nonlinear optimization problems of the form
\begin{equation}
\label{eqn:mani_optimization}
\min_{\bm{P}\in\Manifold}{J(\bm{P})} 
\end{equation}
where $J$ is the loss function and the search space of the parameters (\textit{i.e.} $\bm{P}$) is defined over a smooth Riemannian manifold $\Manifold$ \cite{absil2009optimization}.
\end{definition}

The Euclidean GD-based methods can not be used to solve the optimization problem of Eqn.~\eqref{eqn:mani_optimization}, because they do not calculate the derivatives of the loss function with respect to the manifold geometry. Moreover, any translation between the current and next points on the gradient descent direction should also respect the geometry of Riemannian spaces.
To tackle these challenges, one popular choice is to resort to gradient-based Riemannian optimization algorithms that exploit the geometry of Riemannian manifolds by making use of several Riemannian operations including \textit{orthogonal projection}, \textit{retraction} and \textit{parallel transport}.


\begin{definition}[Orthogonal projection]
For any point $\textit{\textbf{P}}\in \Manifold$, the orthogonal projection operator $\pi_\textit{\textbf{P}}:\mathbb{R}^n\rightarrow T_\textit{\textbf{P}}\Manifold$ transforms an Euclidean gradient vector to Riemmanian gradient (a vector setting on the tangent space $T_\textit{\textbf{P}}\Manifold$).
\end{definition}
\begin{definition}[Exponential map and Retraction]
An exponential map, $\textrm{Exp}_{\textit{\textbf{P}}}(\cdot)$, maps a tangent vector $\textit{\textbf{v}}\in T_{\textit{\textbf{P}}} \Manifold$ to a manifold $\Manifold$. $\textrm{Exp}_{\textit{\textbf{P}}}(t \textit{\textbf{v}})$ represents the corresponding geodesic $\gamma(t):t\in [0,1]$, such that $\gamma(0) = \textit{\textbf{P}}$, $\dot{\gamma} (0) = \textit{\textbf{v}}$ on the manifold. However, evaluating the exponential map is computationally expensive. Retraction operation $R_{\textit{\textbf{P}}}:T_{\textit{\textbf{P}}} \Manifold \rightarrow \Manifold$ is usually used as a more efficient alternative that provides an estimation of exponential map.     
\end{definition}
\begin{definition}[Parallel transport]
The parallel transport operation $\Gamma_{\textit{\textbf{P}} \rightarrow \textit{\textbf{Q}}} : T_{\textit{\textbf{P}}} \Manifold \rightarrow T_{\textit{\textbf{Q}}} \Manifold$, takes a tangent vector $\textit{\textbf{v}} \in T_{\textit{\textbf{P}}} \Manifold$ on a point $\textit{\textbf{P}}$ and translates it to the tangent space of another point $\textit{\textbf{Q}}$ along a geodesic curve that connects $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ on the manifold $\Manifold$ and outputs $\textit{\textbf{u}} \in T_{\textit{\textbf{Q}}} \Manifold$. Parallel transport preserves the norm of the vector during this process and makes sure that the intermediate vectors are always lying on a tangent space. In practice,
if $\Gamma_{\textit{\textbf{P}}\rightarrow \textit{\textbf{Q}}}$ is not known for a given Riemannian manifold or if it is computationally expensive to evaluate, one can, as an approximation, use the orthogonal projection to correct and map tangent vectors between $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ on $\Manifold$ \cite{boothby1986introduction}.
\end{definition}

Based on the above operations, $\textit{\textbf{P}}$ in Eqn.~\eqref{eqn:mani_optimization} is updated by:
\begin{equation}
\label{eqn:optim-update}
\begin{aligned}
\boldsymbol{P}^{(t+1)}&=R_{\boldsymbol{P}^{(t)}}\big(-\alpha \pi_{\boldsymbol{P}^{(t)}}(\nabla J)\big)
\end{aligned}
\end{equation}

where $\alpha$ is the step size and $\big(-\alpha \pi_{\boldsymbol{P}^{(t)}}(\nabla J)\big)$ is the search direction on the tangent space. In Riemannian gradient descent algorithms, search directions are computed by transforming the Euclidean gradient $\nabla J$ to the Riemannian gradient using the orthogonal projection operation. After obtaining the Riemannian gradient on the tangent space, the retraction operation is applied to find the updated Riemannian parameter on manifolds. In other words, the retraction operation is analogous to traversing the manifold along the search direction.
In some gradient-based methods such as Momentum SGD (M-SGD) \citep{qian1999momentum}, it is needed to take the sum of the gradient vectors over time. However, such summation of gradients over time is not a straightforward operation on a Riemannian manifold unless the gradients are \emph{parallely transported} to a common tangent space. Fig.~\ref{fig:manifold-operation} provides a detailed schematic of the various manifold operations as explained above.

\begin{figure*}[t]
\centering
\includegraphics[scale=0.25, keepaspectratio]{Figures/operations.png}
\caption{An Illustrative schematic of various operations required in GD-based optimization on Riemannian manifold. Let $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ represent points on the manifold $\Manifold$ connected by a geodesic shown by the \textbf{\textcolor{electricgreen}{light green dashed}} curve. The tangent spaces at $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$, \textit{i.e.} $T_{\textit{\textbf{P}}} \Manifold$ and $T_{\textit{\textbf{Q}}} \Manifold$ are shown in \textbf{\textcolor{orange}{\textbf{orange}}} color. Vector $\textit{\textbf{v}}_1 \in  T_{\textit{\textbf{P}}} \Manifold$ is the result of the orthogonal projection of the euclidean vector $\textit{\textbf{u}}$ at $\textit{\textbf{P}}$. The retraction operation $\textit{\textbf{R}}\!=\!R_{\textit{\textbf{P}}}(\textit{\textbf{v}}_1)$ is used to move back to the manifold from the tangent space at $\textit{\textbf{P}}$. In a neighborhood of $\textit{\textbf{P}}$, the retraction operation (shown in \textbf{\textcolor{brown}{brown}}) identifies a point on the geodesic. The parallel transport  $\textit{\textbf{v}}_2\!=\!\Gamma_{\textit{\textbf{P}}\rightarrow \textit{\textbf{Q}}}(\textit{\textbf{v}}_1)$ maps $\textit{\textbf{v}}_1 \in T_{\textit{\textbf{P}}} \Manifold$ to $\textit{\textbf{v}}_2 \in T_{\textit{\textbf{Q}}} \Manifold$ by parallely moving across the geodesic (as shown in \textbf{\textcolor{blue(ryb)}{blue dotted}} arrows) connecting \textit{\textbf{P}} and \textit{\textbf{Q}}.}
\label{fig:manifold-operation}
\end{figure*} 


\begin{table*}[]
\centering
\caption{The Required Riemannian operators for Stiefel manifold, where $\text{Sym}(\textit{\textbf{x}})=\frac{1}{2}(\textit{\textbf{x}}+\textit{\textbf{x}}^\top)$ and $\text{uf}(\textit{\textbf{x}})=\textit{\textbf{x}}(\textit{\textbf{x}}^\top\textit{\textbf{x}})^{-\frac{1}{2}}$.}
\label{tab:manifold operations}
\begin{tabular}{|c|c|c|}
\hline

Orthogonal projection $\pi_\textit{\textbf{x}}(\textit{\textbf{u}})$ & Retraction $R_{\textit{\textbf{x}}}(\textit{\textbf{v}})$ & Parallel transport  $\Gamma_{\textit{\textbf{x}} \rightarrow \textit{\textbf{y}}}(\textit{\textbf{w}})$ \\ 
\hline

$\textit{\textbf{u}}-\textit{\textbf{x}} \text{Sym}(\textit{\textbf{x}}^\top\textit{\textbf{u}})$ & $\text{uf}(\textit{\textbf{x}}+\textit{\textbf{v}})$ & $\pi_\textit{\textbf{y}}(\textit{\textbf{w}})$ \\
\hline
\end{tabular}
\end{table*}


==> Sections/Sections/Results.tex <==
\section{Experiments and Results}
\label{Sec-Results}

\subsection{Evaluation Scenarios and Datasets}
We evaluate our proposed method across different few-shot classification tasks. Following the experimental setting provided by \cite{chen2019closer,tabealhojeh2023rmaml}, we address both \emph{single-domain} and \emph{cross-domain} scenarios. In the single-domain experiments, the meta-train, meta-validation, and meta-test tasks are sampled from one dataset, while in the cross-domain scenarios, the meta-test tasks are from a different dataset. Thereby the effect of domain shift in our proposed method is studied in this scenario.

\subsubsection{Single-domain image classification}

To address the single-domain scenario, we conduct two scenarios including object recognition and fine-grained image classification. Mini-ImageNet \citep{ravi2016optimization} is used for object recognition, which includes a subset of 100 classes from the ImageNet dataset \citep{vinyals2016matching} and 600 images sampled from each class. Following the setting provided by Ravi and Larochelle \citep{ravi2016optimization}, the dataset is split into randomly selected 64, 16, and 20 classes for meta-train, meta-validation and meta-test, respectively.

For fine-grained image classification, we use the CUB-200-2011 (CUB) \citep{wah2011caltech} and FC100 \citep{krizhevsky2009learning} datasets. The CUB dataset consists of 11,788 images belonging to 200 different classes of birds. Following the evaluation protocol of \citep{hilliard2018few}, the dataset is randomly divided into the train, validation, and test meta-sets with 100, 50, and 50 classes respectively.
The FC100 dataset is based on the popular object classification dataset CIFAR100 \citep{krizhevsky2009learning} and offers a more challenging few-shot scenario, because of the lower image resolution and using more challenging meta-training/test splits that are separated according to the object superclasses. The dataset contains 100 object classes and each class has 600 samples of 32×32 color images. These 100 classes belong to 20 superclasses. Following the splits proposed by Krizhevsky et al. \citep{oreshkin2018tadam}, meta-training data contain 60 classes from 12 super-classes. Meta-validation and meta-test sets are from 20 classes belonging to 4 super-classes, respectively. Splitting the data according to the 500 super-classes minimizes the information overlap between training and validation/test tasks.

\subsubsection{Cross-domain image classification} 
    One key aspect of few-shot experiments is investigating the domain shift's effect between the meta-train and meta-test datasets on the meta-learning algorithm. For instance, one can observe that the domain gap between the meta-train and meta-test classes of miniImageNet is larger than that of CUB in a word-net hierarchy \citep{miller1995wordnet}. Thus, meta-learning on miniImageNet is more challenging than the CUB dataset. Hence, we also address the cross-domain scenario in our experimental setup. The cross-domain experiment enables us to study the effect of domain shift on our proposed method, although our method was originally developed for single-domain classification.

    Following the scenarios provided by state-of-the-art works \citep{chen2019closer}, we conduct \emph{mini-ImageNet$\rightarrow$CUB} and \emph{Omniglot$\rightarrow$EMNIST} cross-domain experiments. For the \emph{mini-ImageNet$\rightarrow$CUB} experiment, all of the $100$ classes of mini-ImageNet are used as meta-train set, while 50 meta-validation and 50 meta-test classes are sampled from CUB. For \emph{Omniglot$\rightarrow$EMNIST} experiment,
    we follow the setting proposed by Dong and Xing \citep{dong2018domain}, where the non-Latin characters of Omniglot dataset are used as the meta-train classes and the EMNIST dataset \citep{cohen2017emnist} that contains 10-digits and upper and lower case alphabets in English, is used for our meta-validation and meta-test classes. In total, the meta-train set consists of 1597 classes from the Omniglot dataset, while the 62 classes of EMNIST are split into 31 classes for meta-validation and 31 classes for meta-test sets. 


\subsection{Experimental Details}
We use the standard $N\text{-way}$ $k\text{-shot}$ classification setups, in which every task instance contains randomly sampled classifying images from $N$ different categories of the meta-train set. For each class, we sample $k$ instances as our support set and $q$ instances for the query set. For the meta-test phase, we run 600 experiments and report the average classification accuracy and the 95\% confidence interval of these 600 trials as the final result. $N$, $k$, and $q$ are sampled similarly to the meta-train stage. In our experiments, $N$ is set to 5 for all of the experiments across all datasets. %We apply standard data augmentation operations including random crop, left-right flip, and color jitter in the meta-train set, while no such data augmentation strategies are used for meta-validation and meta-test sets. For cross-domain character recognition (Omniglot$\rightarrow$EMNIST) experimental setup, the white-on-black EMNIST data are inverted to black-on-white, as in Omniglot. Moreover, since Omniglot characters are black-and-white, center-aligned and rotation sensitive, we do not use data augmentation in this experiment. 

For mini-ImageNet and CUB datasets, we use a four-layer convolutional backbone (Conv-4) with an input size of $84\times 84$. We also use the ResNet-18 backbone network with an input size of $224\times 224$, while for the Fc100 experiment, we use Conv4 and ResNet12 backbone networks. We also use Conv4 for cross-domain character recognition (\emph{Omniglot$\rightarrow$EMNIST}) experimental setup, while ResNet-18 network is used for \emph{mini-ImageNet$\rightarrow$CUB} experiment.

In all of the experiments across every network backbone, we assume that the parameters of the last fully connected layer of the network are orthonormal and lie on a Stiefel manifold. FORML meta-learns this matrix using the Riemannian operators, as described in Algorithm~\ref{alg-RMAML}. FORML optimizes the parameters of the remaining layers in Euclidean space. All the experiments were performed on a single NVIDIA V100 GPU with a memory capacity of 32GB. 

\subsubsection{Hyper-parameter setups} 
Table~\ref{tab:notations} introduces the notation used for the Steifel and Euclidean hyper-parameters. In the \textbf{single-domain} setup: 
\begin{itemize}
    \item $\alpha$ is set to $0.1$ for experiments with Conv4 backbone architecture, while it is set to $0.01$ for the others. 
    \item $\widehat\eta$ is set to $10^{-3}$ for all experiments with Conv4 backbone architecture.
    \item $\widehat\eta$ is set to $10^{-4}$ for experiments on the CUB and Mini-ImageNet datasets using ResNet-18 backbone architecture.
    \item In FC100 classification experiments, the hyper-parameters setting of Conv4 and ResNet-12 backbones are equal to those of the CUB experiments with Conv4 and ResNet-18, respectively. 
\end{itemize}

Similarly, for the experiments in the \textbf{cross-domain} setup: 
\begin{itemize}
    \item the value of $\alpha$ is set to $0.01$ for mini-ImageNet$\rightarrow$CUB, and is set to $0.05$ and $0.1$ for Omniglot$\rightarrow$EMNIST 1-shot and 5-shot experiments, respectively. 
    \item $\widehat\eta$ for mini-ImageNet$\rightarrow$CUB is set $5\times10^{-4}$, while it is set to $10^{-3}$ and $10^{-4}$ for Omniglot$\rightarrow$EMNIST 1-shot and 5-shot experiments, respectively.
\end{itemize}

For all experiments, the learning rate $\widetilde\eta$ and the weight decay $\lambda_{\widetilde\eta}$ are set to $10^{-3}$ and $0$. Similarly, the value of $\lambda_{\widehat\eta}$ is set to $0$ for experiments with Conv4 backbone architecture, while it is set to $10^{-4}$ for experiments with ResNet-18 architectures. All hyper-parameters are obtained by trial and error and for all experiments, the batch size and the number of inner-level updates for training are always set to 4 and 5, respectively.

\begin{table}[]
\centering
\caption{Notations and descriptions of hyper-parameters for experiments with RMAML.}
\label{tab:notations}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Symbol} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Learning\\ Rate\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Weight\\ Decay\end{tabular}} & \multicolumn{1}{c|}{Parameters} & \multicolumn{1}{c|}{Loop} \\ \hline
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\ \hline
$\alpha$ & $\checkmark$ & $\times$ & \multirow{2}{*}{Stiefel} & \multirow{2}{*}{Inner}  \\
$\lambda_{\alpha}$ & $\times$ & $\checkmark$ &  &  \\ \hline
$\widetilde\eta$ & $\checkmark$ & $\times$ & \multirow{2}{*}{Stiefel} & \multirow{2}{*}{Outer}  \\
$\lambda_{\widetilde\eta}$ & $\times$ & $\checkmark$ &  &  \\ \hline

$\widehat\eta$ & $\checkmark$ & $\times$ & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non\\ Stiefel\end{tabular}} & \multirow{2}{*}{Outer}  \\
$\lambda_{\widehat\eta}$ & $\times$ & $\checkmark$ &  &  \\ \hline

\end{tabular}
\end{table}
% \end{description}

% In the experiments mentioned above, the value of weight decay for the 
\subsubsection{Methods used for comparison}


\subsection{Results for Single-Domain Experiments}

We conduct the standard 5-way 1-shot and 5-shot experiments for single-domain few-shot classification. Table~\ref{tab1: all experiments} presents few-shot classification results for single-domain experiments with different backbone networks, on mini-ImageNet and CUB datasets. Among all the experimental setups, RMAML has a significant improvement over its non-Riemannian counterpart (\textit{i.e} MAML) in terms of classification accuracy (\textit{e.g.} $75.79\pm0.92$ vs $68.42\pm1.07$ for the 1-shot experiment on the CUB dataset using ResNet18 backbone). Moreover, as the depth of the backbone network is increased (Conv4 $\rightarrow$ ResNet18), RMAML either outperforms or achieves comparable results with respect to the other meta-learning methods considered for comparison for both 1-shot and 5-shot experiments.
We also adopt Conv4 and ResNet12 backbones to assess our algorithm against FC100 dataset. As shown in Table~\ref{tab:FC100-exp}, we observe that RMAML improves the few-shot recognition performance on FC100 dataset, compared to its Euclidean counterpart and other methods. 

Compared to its Euclidean counterpart, as it is evident in Tables~\ref{tab1: all experiments} and \ref{tab:FC100-exp}, our proposed algorithm RMAML has remarkably outperformed MAML across all the backbone network architectures for all the single domain experimental setups. A pictorial comparison between RMAML and MAML is shown in Fig.~\ref{fig:MAML vs RMAML} for better understanding. Furthermore, as the depth of the backbone network is increased, MAML fails to improve its results on the CUB dataset due to over-fitting to its training set, while no such over-fitting is observed for RMAML and its performance continues to improve as the networks become deeper. Moreover, one can clearly observe that for experiments on miniImageNet, RMAML outperforms MAML by a significant margin as the depth of the network increases; even though both these methods overfit to the training set for the ResNet-18 backbone.

 \begin{table*}
 \centering
 \caption{A comparison on few-shot classification accuracies between first-order approximation methods in Euclidean space (MAML) and Stiefel manifold (FORML) for mini-ImageNet and CUB datasets against different backbone networks are shown in the last 3 columns. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab1: all experiments}
 \begin{tabular}{lllll}
 %\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|c|l|cccc|}%@{\extracolsep{\fill}}}
 \hline%toprule
 \multicolumn{1}{c}{\textbf{Dataset}}  & \textbf{Method} & \textbf{Conv-4} & \textbf{Conv-6} & \textbf{ResNet-10} %& \textbf{ResNet-18} 
 \\ \hline
 \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 1-shot\end{tabular}} &  MAML (First-Order) \cite{chen2019closer}  & $54.73\pm0.97$ &  $66.26\pm1.05$& $70.32\pm0.99$ %& $68.42\pm1.07$
 \\
 & FORML (ours) & $\bm{58.86\pm0.99}$ & $\bm{67.29\pm0.99}$ & $\bm{70.96\pm0.97}$  %&$\bm{71.68\pm0.99}$
 \\
  \hline%midrule
  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}CUB 5-shot\end{tabular}} & MAML (First-Order) \cite{chen2019closer} & $75.75\pm0.76$& $78.82\pm0.70$& $80.93\pm0.71$  %&$83.47\pm0.62$
  \\
  & FORML (ours) & $\bm{77.93\pm0.95}$& $\bm{79.76\pm0.98}$7 & \bm{$82.45 \pm 0.69$}   %&\bm{$84.76 \pm 0.64$} 
  \\
  \hline%midrule
  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 1-shot\end{tabular}} 
  &MAML (First-Order)\cite{chen2019closer} &$46.47\pm0.82$ &$50.96\pm0.92$& $54.69\pm0.89$ %&$49.61\pm0.92$
  \\
 %& Reptile \cite{nichol2018first} & $47.07\pm0.26$ &  $-$& $-$ & $-$\\
 & FORML (ours) &\bm{$47.89\pm0.80$} & \bm{$51.68\pm0.55$}& \bm{$55.13 \pm 0.88$}  %&\bm{$51.23 \pm 0.89$}
 \\
  \hline%midrule
  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}mini-ImageNet \\ 5-shot\end{tabular}} 
 & MAML (First-Order) \cite{chen2019closer} &$62.71\pm0.71$& $66.09\pm0.71$ &$66.62\pm0.83$ %&$65.72\pm0.77$
 \\
 %& Reptile \cite{nichol2018first}  & $62.74\pm0.38$ &  $-$& $-$ & $-$\\
 & FORML (ours) & \bm{$64.46\pm0.68$} & \bm{$68.12\pm0.88$}& \bm{$68.82\pm0.85$} %&\bm{$67.89\pm0.75$} 
 \\
  \bottomrule
 \end{tabular}
 \end{table*}



\begin{table*}
\centering
\caption{Few-shot classification accuracies for mini-ImageNet and CUB datasets against different backbone networks are shown in the last 4 columns. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab1: all experiments}
\begin{tabular}{lllll}
\hline%toprule
\multicolumn{1}{c}{\textbf{Method}}  & \textbf{Backbone}& \textbf{Manifold} & \textbf{1-shot} & \textbf{5-shot} \\ \hline
MAML (first-0order) \cite{chen2019closer} &Conv4& Euclidean & $46.47\pm0.82$ & $62.71\pm0.71$\\
Reptile \cite{nichol2018first}&Conv4& Euclidean &$47.07\pm0.26$ &$62.74\pm0.38$\\
FORML \cite{nichol2018first}&Conv4& Stiefel &\bm{$47.89\pm0.80$} &\bm{$64.46\pm0.68$}\\

 \bottomrule
\end{tabular}
\end{table*}




\begin{table*}
\centering
\caption{Few-shot classification accuracies for FC100 dataset. All experiments are from 5-way classification learned with data augmentation. The best results are shown in \textbf{bold}.}\label{tab:FC100-exp}
\begin{tabular}{lllll}
\toprule
\textbf{Backbone Networks} & \multicolumn{2}{c}{\textbf{Conv4}} & \multicolumn{2}{c}{\textbf{ResNet12}} \\ 
\cmidrule(r){1-5}
\textbf{Method} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
\cmidrule(r){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-5}
Baseline & $32.48\pm 0.58$ & $47.15 \pm 0.67$ & $38.24 \pm 0.63$ & $56.87 \pm 0.71$ \\
% MatchingNet & $35.36 \pm 0.68$ & $48.36 \pm 0.71$ & $40.85 \pm 0.75$ & $55.70 \pm 0.71$ \\
% ProtoNet &  $34.86 \pm 0.72$ & $48.79 \pm 0.70$ & $40.90\pm 0.73$ & \bm{$57.95\pm 0.70$}\\
% RelationNet & $37.52\pm 0.74$ & $48.94\pm 0.72$ & $37.02\pm 0.79$ & $49.83\pm 0.73$ \\
MAML\cite{chen2019closer} & $36.70\pm 0.83$ & $47.69\pm0.79$ & $40.15\pm0.78$ & $54.13\pm0.77$ \\
FORML (ours) & \bm{$38.82\pm0.72$} & \bm{$49.05\pm0.88$} & \bm{$41.30\pm0.68$} & \bm{$57.35\pm0.84$}  \\ 
\bottomrule

\end{tabular}
\end{table*}
\begin{table*}[t]
\centering
\caption{Supplementary comparison for Few-shot classification results on FC100 dataset. The best results are shown in \textbf{bold}.}\label{tab:further-exp-FC100}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Backbone} & \textbf{1-shot} & \textbf{5-shot} \\ \hline
MetaOptNet~\citep{lee2019meta} & ResNet12 & $41.10\pm0.60$& $55.50\pm0.60$ \\
Arcmax~\citep{afrasiyabi2020associative} & ResNet18 & $40.84\pm0.71$ & $57.02\pm0.63$ \\
MixtFSL~\citep{afrasiyabi2021mixture} & ResNet18 & \bm{$41.50\pm0.67$} & \bm{$58.39\pm0.62$} \\
FORMLL (ours) & ResNet12 & $41.30\pm0.68$ & $57.35\pm0.84$\\ \hline

\end{tabular}
\end{table*}
\subsection{Results for Cross-Domain Experiments}
Table~\ref{tab:cross-exp} shows the results of mini-ImageNet$\rightarrow$CUB and Omniglot$\rightarrow$EMNIST experiments. For 1-shot Omniglot$\rightarrow$EMNIST experiment, RMAML  outperforms all other methods (except the RelationNet method) as shown in Table~\ref{tab:cross-exp}, while still obtaining comparable results to MatchingNet and RelationNet for the 5-shot experiment. Moreover, RMAML has remarkably outperformed MAML by more than $9\%$, in terms of classification accuracy in mini-ImageNet$\rightarrow$CUB experiment.  However, in this experiment one can observe that the Baseline method outperforms all the other methods (including MAML and RMAML) as it is much simpler to adapt to the target domain by learning a new parameterized classifier layer for the Baseline method. On the other hand, meta-learning methods fail to overcome the diverse and significant domain gap between the meta-train and meta-test sets in comparison to Baseline method~\citep{vinyals2016matching, chen2019closer}. Having said that, RMAML still obtains competitive results in terms of classification accuracy against other meta-learning methods. Excluding the Baseline results, RMAML obtains the second best result in 1-shot Omniglot$\rightarrow$EMNIST and 5-shot mini-ImageNet$\rightarrow$CUB  experiments and the third stage in 1-shot Omniglot$\rightarrow$EMNIST experiment. Compared to MAML, our proposed method can achieve results analogous to its Euclidean counterpart, while it can strongly outperforms MAML when deeper backbone network is used. For instance, unlike MAML, RMAML prevents ResNet18 from over-fitting in mini-ImageNet$\rightarrow$CUB experiment. 



\begin{table*}
\centering
\caption{Classification accuracies for \textbf{Omniglot$\rightarrow$EMNIST} and \textbf{mini-ImageNet$\rightarrow$CUB} cross-domain experimental setup.}\label{tab:cross-exp}
\begin{tabular}{llll}
\toprule
 & \multicolumn{2}{l}{\textbf{Omniglot$\rightarrow$EMNIST}} & \textbf{mini-ImageNet$\rightarrow$CUB} \\ 
 \cmidrule(r){2-4}
\textbf{Backbone Networks} & \multicolumn{2}{l}{\textbf{Conv4}} & \multicolumn{1}{l}{\textbf{ResNet18}} \\ 
\midrule

\textbf{Method} & \textbf{1-shot} & \textbf{5-shot} & \textbf{5-shot} \\ \cmidrule(r){1-1}
\cmidrule(r){2-3}
\cmidrule(r){4-4}
Baseline & $63.94\pm0.87$ & $86.00\pm0.59$ & \bm{$65.57\pm0.70$} \\
% MatchingNet & $72.71\pm0.79$ & $87.60\pm0.56$ & $53.07\pm0.74$ \\
% ProtoNet &  $70.43\pm0.80$ & $87.04\pm0.55$ & $62.02\pm0.70$ \\
% RelationNet & \bm{$75.55\pm0.87$} & \bm{$88.94\pm0.54$} & $57.71\pm0.73$ \\
MAML & $72.04\pm 0.83$ & \bm{$88.24\pm0.56$}  & $51.34\pm0.72$ \\
FORML (ours) & \bm{$72.78\pm 0.82$} & $87.41 \pm0.57 $  &  $56.43\pm0.71$ \\ \bottomrule
\end{tabular}
\end{table*}




\subsection{Computational Complexity}\label{subsec:computational-complexity}



==> Sections/preliminaries.tex <==
\section{Preliminaries}
\label{Sec-Preliminaries}

\subsection{Riemannian manifolds}
In this section, we introduce the definition of smooth Riemannian manifolds and the required mathematical operations for applying Gradient Descent (GD) or GD-based optimization algorithms in Riemannian spaces.    
\begin{definition}[Smooth Riemannian manifold]
A smooth Riemannian manifold $\Manifold$ is a locally Euclidean space and can be understood as a generalization of the notion of a surface to higher dimensional spaces \cite{lin2008riemannian}. For each point $\textit{\textbf{P}}\in \Manifold$, the tangent space is denoted by $T_\textit{\textbf{P}}\Manifold$. The tangent space at a point $\textit{\textbf{P}}\in \Manifold$ is a vector space that consists of all vectors that are tangent to $\Manifold$ at $\textit{\textbf{P}}$.
\end{definition}
\begin{definition}[Stiefel manifold]
The Stiefel manifold $St(n,p), n \geq p$, is a Riemannian manifold that is composed of all $n \times p$ orthonormal matrices, i.e. $\{\textbf{P}\in \mathbb{R}^{n \times p}:\textbf{P}^T\textbf{P}=\textbf{I}\}$. 
\end{definition}

\begin{definition}[Manifold optimization]
Manifold optimization refers to nonlinear optimization problems of the form
\begin{equation}
\label{eqn:mani_optimization}
\min_{\bm{P}\in\Manifold}{J(\bm{P})} 
\end{equation}
where $J$ is the loss function and the search space of the parameters (\textit{i.e.} $\bm{P}$) is defined over a smooth Riemannian manifold $\Manifold$ \cite{absil2009optimization}.
\end{definition}

The Euclidean GD-based methods can not be used to solve the optimization problem of Eqn.~\eqref{eqn:mani_optimization}, because they do not calculate the derivatives of the loss function with respect to the manifold geometry. Moreover, any translation between the current and next points on the gradient descent direction should also respect the geometry of Riemannian spaces.
To tackle these challenges, one popular choice is to resort to gradient-based Riemannian optimization algorithms that exploit the geometry of Riemannian manifolds by making use of several Riemannian operations including \textit{orthogonal projection}, \textit{retraction} and \textit{parallel transport}.


\begin{definition}[Orthogonal projection]
For any point $\textit{\textbf{P}}\in \Manifold$, the orthogonal projection operator $\pi_\textit{\textbf{P}}:\mathbb{R}^n\rightarrow T_\textit{\textbf{P}}\Manifold$ transforms an Euclidean gradient vector to Riemmanian gradient (a vector setting on the tangent space $T_\textit{\textbf{P}}\Manifold$).
\end{definition}
\begin{definition}[Exponential map and Retraction]
An exponential map, $\textrm{Exp}_{\textit{\textbf{P}}}(\cdot)$, maps a tangent vector $\textit{\textbf{v}}\in T_{\textit{\textbf{P}}} \Manifold$ to a manifold $\Manifold$. $\textrm{Exp}_{\textit{\textbf{P}}}(t \textit{\textbf{v}})$ represents the corresponding geodesic $\gamma(t):t\in [0,1]$, such that $\gamma(0) = \textit{\textbf{P}}$, $\dot{\gamma} (0) = \textit{\textbf{v}}$ on the manifold. However, evaluating the exponential map is computationally expensive. Retraction operation $R_{\textit{\textbf{P}}}:T_{\textit{\textbf{P}}} \Manifold \rightarrow \Manifold$ is usually used as a more efficient alternative that provides an estimation of exponential map.     
\end{definition}
\begin{definition}[Parallel transport]
The parallel transport operation $\Gamma_{\textit{\textbf{P}} \rightarrow \textit{\textbf{Q}}} : T_{\textit{\textbf{P}}} \Manifold \rightarrow T_{\textit{\textbf{Q}}} \Manifold$, takes a tangent vector $\textit{\textbf{v}} \in T_{\textit{\textbf{P}}} \Manifold$ on a point $\textit{\textbf{P}}$ and translates it to the tangent space of another point $\textit{\textbf{Q}}$ along a geodesic curve that connects $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ on the manifold $\Manifold$ and outputs $\textit{\textbf{u}} \in T_{\textit{\textbf{Q}}} \Manifold$. Parallel transport preserves the norm of the vector during this process and makes sure that the intermediate vectors are always lying on a tangent space. In practice,
if $\Gamma_{\textit{\textbf{P}}\rightarrow \textit{\textbf{Q}}}$ is not known for a given Riemannian manifold or if it is computationally expensive to evaluate, one can, as an approximation, use the orthogonal projection to correct and map tangent vectors between $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ on $\Manifold$ \cite{boothby1986introduction}.
\end{definition}

Based on the above operations, $\textit{\textbf{P}}$ in Eqn.~\eqref{eqn:mani_optimization} is updated by:
\begin{equation}
\label{eqn:optim-update}
\begin{aligned}
\boldsymbol{P}^{(t+1)}&=R_{\boldsymbol{P}^{(t)}}\big(-\alpha \pi_{\boldsymbol{P}^{(t)}}(\nabla J)\big)
\end{aligned}
\end{equation}

where $\alpha$ is the step size and $\big(-\alpha \pi_{\boldsymbol{P}^{(t)}}(\nabla J)\big)$ is the search direction on the tangent space. In Riemannian gradient descent algorithms, search directions are computed by transforming the Euclidean gradient $\nabla J$ to the Riemannian gradient using the orthogonal projection operation. After obtaining the Riemannian gradient on the tangent space, the retraction operation is applied to find the updated Riemannian parameter on manifolds. In other words, the retraction operation is analogous to traversing the manifold along the search direction.
In some gradient-based methods such as Momentum SGD (M-SGD) \citep{qian1999momentum}, it is needed to take the sum of the gradient vectors over time. However, such summation of gradients over time is not a straightforward operation on a Riemannian manifold unless the gradients are \emph{parallely transported} to a common tangent space. Fig.~\ref{fig:manifold-operation} provides a detailed schematic of the various manifold operations as explained above.

\begin{figure}[t]
\centering
\includegraphics[scale=0.25, keepaspectratio]{Figures/operations.png}
\caption{An Illustrative schematic of various operations required in GD-based optimization on Riemannian manifold. Let $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$ represent points on the manifold $\Manifold$ connected by a geodesic shown by the \textbf{\textcolor{electricgreen}{light green dashed}} curve. The tangent spaces at $\textit{\textbf{P}}$ and $\textit{\textbf{Q}}$, \textit{i.e.} $T_{\textit{\textbf{P}}} \Manifold$ and $T_{\textit{\textbf{Q}}} \Manifold$ are shown in \textbf{\textcolor{orange}{\textbf{orange}}} color. Vector $\textit{\textbf{v}}_1 \in  T_{\textit{\textbf{P}}} \Manifold$ is the result of the orthogonal projection of the euclidean vector $\textit{\textbf{u}}$ at $\textit{\textbf{P}}$. The retraction operation $\textit{\textbf{R}}\!=\!R_{\textit{\textbf{P}}}(\textit{\textbf{v}}_1)$ is used to move back to the manifold from the tangent space at $\textit{\textbf{P}}$. In a neighborhood of $\textit{\textbf{P}}$, the retraction operation (shown in \textbf{\textcolor{brown}{brown}}) identifies a point on the geodesic. The parallel transport  $\textit{\textbf{v}}_2\!=\!\Gamma_{\textit{\textbf{P}}\rightarrow \textit{\textbf{Q}}}(\textit{\textbf{v}}_1)$ maps $\textit{\textbf{v}}_1 \in T_{\textit{\textbf{P}}} \Manifold$ to $\textit{\textbf{v}}_2 \in T_{\textit{\textbf{Q}}} \Manifold$ by parallely moving across the geodesic (as shown in \textbf{\textcolor{blue(ryb)}{blue dotted}} arrows) connecting \textit{\textbf{P}} and \textit{\textbf{Q}}.}
\label{fig:manifold-operation}
\end{figure} 




